HeteSpaceyWalk: A Heterogeneous Spacey Random Walk for Heterogeneous Information Network Embedding

Heterogeneous information network (HIN) embedding has gained increasing interests recently. However, the current way of random-walk based HIN embedding methods have paid few attention to the higher-order Markov chain nature of meta-path guided random walks, especially to the stationarity issue. In this paper, we systematically formalize the meta-path guided random walk as a higher-order Markov chain process, and present a heterogeneous personalized spacey random walk to efficiently and effectively attain the expected stationary distribution among nodes. Then we propose a generalized scalable framework to leverage the heterogeneous personalized spacey random walk to learn embeddings for multiple types of nodes in an HIN guided by a meta-path, a meta-graph, and a meta-schema respectively. We conduct extensive experiments in several heterogeneous networks and demonstrate that our methods substantially outperform the existing state-of-the-art network embedding algorithms.

==> v5 - for arxiv/conclusion.tex <==
\section{Conclusions}\label{sec:conclu}
%In this paper, we formalize a higher-order Markov chain to characterize the transition probabilities of the random walk over HIN, and propose a heterogeneous personalized spacey random walk strategy to improve the HIN embedding problem. 
%As a result of introducing higher-order Markov chain, we are able to compute the stationary distribution of nodes for the random walk, and can use the stationary distribution to supervise the HIN embedding.
%In addition, our framework can be used for arbitrary meta-paths since there is no restriction of the start and end nodes should be of the same type.
%Besides the meta-path guided random walk, we also introduce a second-order meta-schema proximity which can incorporate multiple meta-paths together to conduct the random walk. 
% In this paper, we formalize a higher-order Markov chain to characterize the transition probabilities of the meta-path constrained random walk over HINs, and propose a heterogeneous personalized spacey random walk strategy (called {\it HeteSpaceyWalk}) to efficiently generate high-quality heterogeneous neighborhood, 
% %which is based on a solid mathematical foundation.
% which is mathematically guaranteed to attain the same unique limiting stationary distribution as the normal meta-path based higher-order Markovian random walk.
% We further develop a scalable HIN embedding algorithm: {\it SpaceyMetapath}, which is able to efficiently and effectively produce semantically meaningful embeddings for multiple types of nodes in an HIN guided by an arbitrary meta-path.
% Besides,
% we also develop two scalable HIN embedding algorithms by extending the {\it SpaceyMetapath} from a meta-path to a meta-graph or a meta-schema, which can incorporate more complex structures and richer semantics in an HIN.
% %Experimental results on node classification and link prediction on four heterogeneous networks show that our proposed algorithms consistently and significantly outperform the existing state-of-the-art network embedding algorithms.
% We conduct extensive experiments 
% % in four heterogeneous networks 
% and demonstrate that our methods consistently outperform the existing state-of-the-art network embedding algorithms.
% Experimental results show that our methods are able to achieve better performance with smaller walk-times and walk-length.
%In the future, we plan to extend our embedding algorithm to other HIN datasets. Moreover, it would be very interesting to further study the theoretical analysis of the personalized spacey random walk for mera-schema based HIN embedding.


In this paper, we propose a heterogeneous personalized spacey random walk strategy to efficiently generate heterogeneous neighborhood, which is based on a solid mathematical foundation. We further develop a scalable HIN embedding algorithms {\it SpaceyMetapath} to efficiently and effectively produce node embeddings in an HIN guided by an arbitrary meta-path.
We also develop two scalable HIN embedding algorithms by extending the {\it SpaceyMetapath} from a meta-path to a meta-graph or a meta-schema.
Experimental results show that our methods are able to achieve better performance with smaller walk-times and walk-length.


==> v5 - for arxiv/definition.tex <==


% \section{Preliminaries}
\section{Problem Definition}\label{sec:problem-definition}
In this section, we introduce the  formulation of the heterogeneous information network embedding problem.
We first define several key concepts related to HINs as follows~\cite{sun2012mining}.
\vspace{-0.05in}
\begin{definition}\label{def:HIN}
{\it \textbf{Heterogeneous Information Network} (HIN).
An information network is defined as a directed graph ${\mathcal G} = ({\mathcal V}, {\mathcal E})$ with an entity type mapping $\phi$: ${\mathcal V} \to \mathcal A$ and a relation type mapping $\psi$: ${\mathcal E} \to \mathcal R$, where ${\mathcal V}$ denotes the entity set, ${\mathcal E}$ denotes the relation set, $\mathcal A$ denotes the entity type set, and $\mathcal R$ denotes the relation type set. 
When the number of entity types $|\mathcal A|>1$ or the number of relation types $|\mathcal R|>1$, the network is called a heterogeneous information network.
Otherwise, it is called a homogeneous information network.}
\end{definition}
\vspace{-0.05in}
%The major difference between an HIN and traditional graphs or networks is that an HIN has multi-typed entities and relations~\cite{ShiLZSY17}.
The meta-schema (or network-schema) provides a high-level description of a given heterogeneous information network.
%Given an HIN, we can further use  meta-schema to provide  a high-level description
\vspace{-0.05in}
\begin{definition}\label{def:meta_schema}
{\it \textbf{Meta-schema}.
Given an HIN ${\mathcal G} = ({\mathcal V}, {\mathcal E})$ with the entity type mapping $\phi$: ${\mathcal V} \to \mathcal A$ and the relation type mapping $\psi$: $\mathcal E \to \mathcal R$,
the meta-schema (or network-schema) for network $\mathcal G$, denoted as $\mathcal T_{\mathcal G} = (\mathcal A, \mathcal R)$, is a graph with entity types as nodes from $\mathcal A$ and relation types as edges from $\mathcal R$.
}
\end{definition}
\vspace{-0.05in}
%An illustrative  heterogeneous scholar network and its meta-schema are shown in Figure~\ref{Fig:A_HIN}(a) and Figure~\ref{Fig:A_HIN}(b), which consists of three entity types: {\it Author}(A), {\it Paper}(P), and {\it Venue}(V), and two relationship types: an author {\it writes} a paper, and a paper is {\it published} in a venue.
Another important concept is the meta-path~\cite{Sun2011a} which defines relationships between entities at the schema level.
\vspace{-0.05in}
\begin{definition}\label{def:meta_path}
{\it \textbf{Meta-path}.
A meta-path $\mathcal P$ is a path defined on the graph of meta-schema $\mathcal{T}_{\mathcal G} = (\mathcal A, \mathcal R)$, with the form of a sequence of node types $\it A_1, A_2,...,A_{L+1}$ and/or relation types $\it R_1, R_2,...,R_L$:
%\begin{equation*}
%{\it A_1  \xrightarrow{R_1} A_2 \xrightarrow{R_2}  \dots \xrightarrow{R_L} A_{L+1}},
%\end{equation*}
${\it A_1  \xrightarrow{R_1} A_2 \xrightarrow{R_2}  \dots \xrightarrow{R_L} A_{L+1}}$ (or $\mathcal P = {\it (A_1\to A_2\to \ldots \to A_{L+1})}$ when there is no ambiguity),
which defines a composite relation $R = R_1 \cdot R_2 \cdot \ldots \cdot R_L$ between types $A_1$ and $A_{L+1}$, where $\cdot$ denotes relation composition operator, and $L$ is the length of $\mathcal P$.
}
\end{definition}
\vspace{-0.05in}
%For simplicity, we use type names connected by ``$\to$'' to denote the meta-path when there are no multiple relations between a pair of types: $\mathcal P = {\it (A_1\to A_2\to \ldots \to A_{L+1})}$.
We call a path $p \!=\! (v_1\!\to\! v_2\!\to\! \ldots\! \to\! v_{L+1})$ between $v_1$ and $v_{L+1}$ in network $\mathcal{G}$ follows the meta-path $\mathcal P$, if $\forall l, \phi(v_l) \!=\! A_l$ and each edge
$e_l \!=\! \langle v_l,v_{l+1} \rangle$ belongs to each relation type $R_l$ in $\mathcal P$.
We call $p$ as a {\it path instance} of $\mathcal P$, denoted as $p \!\in \!\mathcal P$.
% $R_l^{-1}$ represents the reverse order of relation $R_l$.
%Different meta-paths carry different semantics. For example, as illustrated in Figure~\ref{Fig:A_HIN}(c), the meta-path ``{\it Author$\to$Paper$\to$Author} (APA)'' expresses the information ``Two authors co-author a  paper", and  the meta-path ``{\it Author$\to$Paper$\to$Venue$\to$Paper$\to$Author} (APVPA)'' expresses the information ``Two authors write papers at the same venue".
%To measure the semantics % information 
%of different meta-paths, the concept of commuting  matrix~\cite{Sun2011a} is defined as follows.
%\begin{definition}
%	\label{def:commuting_metapath}
%	{\it \textbf{Commuting Matrix of the Meta-path}. 
%		A commuting matrix ${\bf M}_{\mathcal P}$ for a meta-path $\mathcal P = {\it (A_1\to A_2\to \ldots \to A_{L+1})}$ is defined as $ {\bf M}_{\mathcal P} = {\bf W}_{A_1A_2} \cdot {\bf W}_{A_2A_3}\cdot \ldots \cdot{\bf W}_{A_{L}A_{L+1}}$,
%		where ${\bf W}_{A_lA_{l+1}}$ is the adjacency matrix between types $ A_l$ and $ A_{l+1}$.
%		Each entry ${\bf M}_{\mathcal P}(v_i,v_j)$ represents the number of path instances between $v_i$ and $v_j$ following $\mathcal P$, where $\phi(v_i)=A_1$ and  $\phi(v_j)=A_{L+1}$.
%	}
%\end{definition}
% \vspace{-0.04in}
%The commuting matrix provides a general count measure for meta-path based semantic similarity. 
%For example, for author similarity based on meta-path ``APA,'' which simply gives us a commuting matrix ${\bf M}_{{\mathcal P}_{APA}}={\bf W}_{AP} {\bf W}_{AP}^T$, where ${\bf W}_{AP}$ is the author-paper co-occurrence matrix.
%Following the ``APA'' based semantically meaningful information, ${\bf M}_{{\mathcal P}_{APA}}(v_i,v_j)$ represents  the number of co-authored papers between $v_i$ and $v_j$, i.e., ${\bf M}_{{\mathcal P}_{APA}}$ distinguishes whether two authors are similar if they co-author many papers.
Besides the meta-path, 
%people have also found that 
the meta-graph (or meta-structure) is also very useful
which captures complex semantics by integrating multiple meta-paths
~\cite{FangLZWCL16,HuangZCSML16}.
\vspace{-0.05in}
\begin{definition}\label{def:meta_graph}
	{\it \textbf{Meta-graph}.
		A meta-graph (or meta-structure) is a directed acyclic graph $\mathcal{T}_{\mathcal S} \!=\! (\mathcal A_S, \mathcal R_S)$ defined on the given HIN schema $\mathcal{T}_{\mathcal G} \!= \!(\mathcal A, \mathcal R)$, %where each node is an entity type and each edge is a relation type in  $\mathcal{T}_{\mathcal G}$, i.e., 
		where ${\mathcal A_S} \!\subseteq \!{\mathcal A}$ and ${ \mathcal R_S} \!\subseteq\! {\mathcal R}$.
		In general, a meta-graph has only a single source entity type $A_s$ (i.e., with 0 in-degree) and a single target entity type $A_t$  (i.e., with 0 out-degree).
		Specially, we call the meta-graph $\mathcal{T}_{\mathcal S} $ with  $A_s\!=\!A_t$ as a {\it \textbf{recursive meta-graph}} because it can be recursively extended by tail-head concatenation.
	}
\end{definition}
% Compared with single meta-path, the meta-graph can capture more complex semantics by integrating multiple meta-paths.
% Figure~\ref{Fig:A_HIN}(d) shows an illustrative meta-graph defined on a scholar network,
% which expresses the information %``Two authors write their papers containing the same terms and published in the same venue."
% ``Two authors share the same co-author and write papers in the same venue."
\vspace{-0.05in}
As an illustration, Figure~\ref{Fig:A_HIN} shows a heterogeneous network and its meta-schema, as well as the meta-paths and meta-graphs defined at the schema level.
Finally, by considering an HIN as an input, we formally define the problem of HIN embedding as follows.
\vspace{-0.05in}
\begin{definition}
{\it
\textbf{Heterogeneous Information Network Embedding}.
Given a heterogeneous information network, denoted as a graph ${\mathcal G} = ({\mathcal V}, {\mathcal E}; \mathcal A, \mathcal R)$.
Embedding is to learn a function ${\mathnormal f}:{\mathcal V} \to {\mathbb R}^d$ that
projects each node $v \in {\mathcal V}$ to a 
vector in a d-dimensional latent space ${\mathbb R}^d$, $d \ll |{\mathcal V}|$ that are able to capture the structures and semantics of multiple types of nodes and relationships.
}
\end{definition}

%In general, the output of the embedding problem on HIN is the representations matrix $\bf X$, with the $v^{th}$ row, a d-dimensional vector ${\bf X}_v$, corresponding to the representation of node $v$.
%Note that, although there are different types of nodes in ${\mathcal V}$, their representations are mapped into the same latent space.
% The learned node representations can benefit various heterogeneous network mining tasks.
%For example, the embedding vector of each node can be used as the feature input of node classification, clustering, and similarity search tasks.






==> v5 - for arxiv/experiments.tex <==

\begin{figure*}
	\vspace{-0.2in}
	\setlength{\abovecaptionskip}{-0.1cm}
	\setlength{\belowcaptionskip}{-0.2cm}
	\centering
	\subfigure[\small ACM]{
		\label{Fig:ACM_dataset}
		\includegraphics[width=0.23\textwidth]{resources/ACM}
	}
	%     \hfill
%	\hspace{0.1in}
	%    \vspace{0.0in}
	\subfigure[\small DBLP]{
		\label{Fig:DBLP_dataset}
		\includegraphics[width=0.23\textwidth]{resources/DBLP}
	}
%	\hspace{-0.1in}
	%    \vspace{0.in}
	\subfigure[\small Douban]
	{\label{Fig:Douban_dataset}
		\includegraphics[width=0.24\textwidth]{resources/Douban}
	}
	%     \hfill
%	\hspace{0.1in}
	%    \vspace{0.in}
	\subfigure[\small Yelp]
	{\label{Fig:YELP_dataset}
		\includegraphics[width=0.23\textwidth]{resources/YELP}
	}
	% \includegraphics[width=0.4\textwidth]{walk-times-author}
	\caption{\small The meta-schema, meta-paths, and meta-graphs of each dataset used in the experiments.}
	\label{Fig:datasets}
	\vspace{-0.1in}
\end{figure*}


%\vspace{-0.1in}
\section{Experiments}\label{sec:experiments}
In this section, we show the experimental results.
% Code and data to reproduce our results will be available for the camera-ready version due to the double-blind review policy.
\vspace{-0.1in}
\subsection{Datasets}
\label{sec:dataset}
Here we use the following four heterogeneous networks:

%$\bullet$ \textbf{AMiner:}
% AMiner Computer Science (CS) dataset~\cite{tang2008arnetminer} consists of 1,693,531 computer scientists and 3,194,405 papers from 3,883 computer science venues (both conferences and journals) held until 2016. 
%We use the AMiner Heterogeneous Collaboration Network constructed by ~\cite{YuxiaoDong2017}, in which there are three types of nodes: authors (A), papers (P), and venues (V), and two types of relations: authors {\it writes} papers (A--P), and papers {\it published} in venues (P-V).
%% The links represent different types of relationships among three sets of nodes--such as collaboration relationships on a paper.

%$\bullet$ \textbf{DBIS:}
%The Database and Information Systems (DBIS) dataset is a subset of DBLP\footnote{\url{http://dblp.uni-trier.de/xml/}}, constructed by Sun et al~\cite{Sun2011a}, which contains 464 venues (V), their top-5000 authors (A) and 72,902 corresponding publications (P), and two similar relationships as AMiner has.
%% We also construct the heterogeneous collaboration networks from DBIS wherein a link may connect two authors, one author and one paper, as well as one paper and one venue. 

% $\bullet$ \textbf{DBLP:}
%is a bibliographic dataset in computer science.
%We extract papers published in 20 conferences of 4 research fields to form a network. The network includes papers (P), authors (A) and venues (V) as nodes, and authorships (P-A), papers’ venues (P-V) as edges.

 $\bullet$ \textbf{ACM:}
 The ACM dataset~\cite{shi2014hetesim} % was downloaded from ACM  digital library\footnote{\url{http://dl.acm.org/}}  in June 2010, which 
 contains 196 venues (V), 12,499 papers (P), 1,533 terms (T), %after removing stop words in the paper titles and abstracts, 
 17,431 authors (A), and 1,804 author affiliations (F).
% All these papers are labeled with the ACM %category (i.e., subjects).
% subjects.
% The papers and authors are labeled with the ACM subjects.
% After removing the subjects with less than 10 papers, we get 33 subjects and 12,225 labeled papers.
% We further use these papers to assign each author to the category with the majority of his/her publications.
The  meta-schema of  ACM  dataset is shown  in Figure~\ref{Fig:ACM_dataset}.

 $\bullet$ \textbf{DBLP:}
%  The DBLP dataset~\cite{shi2014hetesim} % is a sub-network collected from DBLP website\footnote{\url{http://dblp.uni-trier.de/xml/}}, which
%  includes 20 major conferences from four related areas.
% %  i.e., database, data mining, machine learning, and information retrieval.
The dataset contains 14,376 papers (P), 20 conferences (C), 14,475 authors (A), and 8,920 terms (T).
% In the dataset, 4,057 authors, 20 conferences, and 100 papers are labeled with one of the four research areas.
The meta-schema of DBLP dataset is shown in Figure~\ref{Fig:DBLP_dataset}.

 $\bullet$ \textbf{Douban:}
The Douban dataset~\cite{shi2015semantic} %is a sub-network collected from Douban website\footnote{\url{http://movie.douban.com/}}, which 
 contains 13,367 users (U), 12,677 movies (M), 2,753 groups (G), 349 locations (L), 2,449 directors (D), and 6,311 actors (A).
%  All of the movies are labeled with category (i.e., movie types).
%  After removing the categories with less than 10 movies, we get 28 categories and 12,664 labeled movies.
%  Furthermore, we also get the category of each user, director and actor by using his/her participating movies.
The meta-schema of Douban dataset is shown in Figure~\ref{Fig:Douban_dataset}.
 
  $\bullet$ \textbf{Yelp:}
  The Yelp dataset~\cite{shi2015semantic} %is from the Yelp challenge dataset\footnote{\url{http://www.yelp.com/dataset_challenge/}}, which 
 contains 16,239 users (U), 14,284 businesses (B), 47 cities (C), and 11 compliments (O).
%  All of the businesses are labeled with its category, and
%  we get 77 categories and 14,025 labeled businesses after removing the categories with less than 10 businesses.
The meta-schema of Yelp dataset is shown in Figure~\ref{Fig:YELP_dataset}.



%For each dataset, we construct a corresponding heterogeneous network where entities (A, V, P) as nodes and relations (A--P, P--V) as edges.
%Then we follow~\cite{YuxiaoDong2017} to match the eight categories\footnote{The eight categories are: Computational Linguistics, Computer Graphics, Computer Networks and Wireless Communication, Computer Vision and Pattern Recognition, Computing Systems, Databases and Information Systems, Human Computer Interaction, Theoretical Computer Science.} of venues in Google Scholar\footnote{\url{https://scholar.google.com/citations?view_op=top_venues\&hl=en\&vq=eng}} with those in AMiner and DBIS datasets to get labeled venues.
%For each author, we assign him/her a category with the majority of his/her publications in the labeled venues, and a tie is resolved by random selection among the possible categories.

%The dataset statistics are summarized in Table~\ref{tab:data-statistic}.

%\begin{table}
%\caption{Dataset Statistics: ``\#term'' means the total number of the term, and the figure within parenthesis is the labeled number of corresponding term.\label{tab:data-statistic}}\small
%% \vspace{-0.1in}
%\centering
%\begin{tabular}{ccccc}
%\toprule
%Dataset& \#Paper & \#Author & \#Venue & \#Category\\
%\midrule
%AMiner & 3,194,405 & 1,693,531 (246,678) & 3,883 (133)& 8 \\
%DBIS & 72,902 & 60,694 (29,492) & 464 (35) & 8 \\
%\bottomrule
%\end{tabular}
%% \vspace{-0.05in}
%\end{table}



\vspace{-0.2cm}
\subsection{Experimental Settings}
\label{sec:exp_settings}
We compare the following state-of-the-art homogeneous and heterogeneous network embedding methods.

% homogeneous network representation learning methods (DeepWalk, LINE, Node2vec) and state-of-the-art heterogeneous network representation learning methods (PTE, Metapath2vec).

$\bullet$ \textbf{DeepWalk}~\cite{PerozziAS14} is a recently proposed homogeneous network embedding model, which learns $d$-dimensional node vectors by capturing the contextual information via uniform random walks.
% In our experiment settings, we ignore the heterogeneity and directly feed the HINs for embedding. We use default training settings, i.e., window size $w = 5$ and length of random walk $l = 40$.

$\bullet$ \textbf{LINE}~\cite{TangQWZYM15} 
is a method that preserves first-order and second-order proximities between nodes separately.
%learns node vectors by considering 1st- and 2nd-order proximities separately.
We use the suggested version to learn two $d/2$-dimensional vectors (one for each-order) and then concatenate them.
% We use the advanced version of LINE by considering both the 1st- and 2nd-order of node proximity;
% For each node, it computes two vectors, one for the first-order and one for the second-order proximities separately and then concatenates them. 
%We use two $d/2$-dimensional vector representations for the first-order and second-order proximities, and then concatenate them to form a $d$-dimensional node vector.
% Same as DeepWalk, we directly feed the HINs for embedding, and use the default training settings. 

%$\bullet$ \textbf{Node2vec}~\cite{GroverL16} is generalized from DeepWalk, which learns $d$-dimensional node vectors by capturing node pairs within $w$-hop neighborhood via parameterized random walks.
%Here we use $p=4$ and $q=1$ in node2vec for comparison, as suggested.

$\bullet$ \textbf{PTE}~\cite{Tang2015PTE} 
%decomposes an HIN to a set of bipartite networks by edge types, and learns $d$-dimensional node vectors by capturing 1-hop neighborhood of the resulting bipartite networks.
is an extension of LINE for heterogeneous network embedding, which decomposes an HIN to a set of bipartite networks by edge types.

% $\bullet$ \textbf{HIN2Vec}~\cite{fu2017hin2vec}

$\bullet$ \textbf{Metapath2vec}~\cite{YuxiaoDong2017} is the current state-of-the-art network embedding method for HINs, which formalizes meta-path-based random walks to generate heterogeneous neighborhood 
%of a node 
and then leverages a heterogeneous skipgram model to perform node embeddings.

$\bullet$ \textbf{Metagraph2vec}~\cite{zhang2018metagraph2vec} uses a meta-graph to guide the generation of random walks and to learn latent embeddings for multiple types of nodes in HINs.



% \subsection{Experimental Settings}
% All of our experiments were run on $K80$ GPUs. The operating system and software platforms are Debian 7.0, TensorFlow r0.12 and Python 3.4.
%For all embedding methods, we use the same dimensionality of node vectors $d=128$ for a trade-off between the computational time and accuracy.
%In the experiment, all the hyperparameters of both baseline methods and our methods are tuned to perform the best on the validation set.
We evaluate the quality of embedding vectors learned by different methods over two classical heterogeneous network mining tasks:
% including multi-label node classification, %node clustering, 
multi-label node classification and link prediction. %and visualization.
% To ensure the significance of the results, we repeat each experiment ten times independently and use the mean values as the reporting results. 
%We also try our best to tune the model training for both our methods and baseline methods.
%As a result, all the experiments of each method produce best results to our best efforts.
%To compare the performance, we empirically set the common hyperparameters as follows: 
For the common hyperparameters, we set
learning rate $lr\!=\!0.025$,  %the size of 
negative samples $m\!=\!5$, and the embedding dimension $d\!=\!128$ for a trade-off between the computational time and accuracy.
For random walk based methods, 
we set walk times per node $t\!=\!20$, walk length of each walk $l\!=\!320$, neighborhood size $w\!=\!10$.
Specially, for our proposed {\it SpaceyMetapath}, {\it SpaceyMetagraph}, and {\it SpaceyMetaschema}, we set the personalized probability $\alpha\!=\!0.8$.
For LINE and PTE, we set the total number of samples as 100 million.
For meta-path driven (Metapath2vec, SpaceyMetapath) and meta-graph driven (Metagraph2vec, SpaceyMetagraph) methods,
we survey most of the meta-path/meta-graph based work and empirically use some meta-paths and meta-graphs (which has been proven to be the most commonly effectively used schemes to extract heterogeneous semantics~\cite{Sun2011a,shi2014hetesim,YuxiaoDong2017,zheng2017recommendation,zhang2018metagraph2vec}).
The selected meta-paths and meta-graphs of each dataset %used in the experiments 
are shown in Figure~\ref{Fig:datasets}.





%For meta-path driven embedding methods, we empirically use the meta-path ``APVPA'' (which has been proven to be the best meta-path on scholar networks~\cite{Sun2011a,YuxiaoDong2017}) to guide embedding in the heterogeneous academic networks, which represents the heterogeneous semantics of authors publishing papers at the same venues.
%For the meta-schema driven embedding, we use the meta-paths shown in Figure~\ref{fig:metaschema-sim}.
%For each method, we evaluate the quality of the learned representations over two classical heterogeneous network mining tasks, including multi-class node classification and clustering.

%To ensure the significance of the results, we repeat each experiment ten times independently and use the mean value as the reporting result. 
%We also try our best to tune the model training for both our methods and baseline methods. As a result, all the experiments of each method produce best results to our best efforts.

%\begin{table}[!htb]
%\caption{\label{Tab:classify-author-AMiner}Experimental results of author node classification on the AMiner dataset.}\small
%\vspace{-0.1in}
%\centering
%% \renewcommand\arraystretch{0.5}
%\begin{tabular}{ccccccc}
%\toprule
%Macro-F1 & 10\% & 30\% & 50\% & 70\% & 90\% \\
%\midrule
%DeepWalk & 0.8534 & 0.8584 & 0.8587 & 0.8585 & 0.8588\\
%Node2vec & 0.8665 & 0.8714 & 0.8733 & 0.8738 & 0.8748\\
%LINE & 0.8886 & 0.8921 & 0.8929 & 0.8936 & 0.8934\\
%\midrule
%PTE & 0.8940 & 0.8982 & 0.8990 & 0.8999 & 0.9005\\
%Metapath2vec & 0.9262 & 0.9303 & 0.9314 & 0.9316 & 0.9320\\
%PMSW-metapath & 0.9390 & 0.9462 & 0.9472 & 0.9473 & 0.9485\\
%\midrule
%PMSW-metaschema & {\bf 0.9429} & {\bf 0.9575} & {\bf 0.9598} & {\bf 0.9597} & {\bf 0.9604}\\
%\toprule
%Micro-F1& 10\% & 30\% & 50\% & 70\% & 90\% \\
%\midrule
%DeepWalk & 0.8684 & 0.8727 & 0.8733 & 0.8733 & 0.8739\\
%Node2vec & 0.8731 & 0.8773 & 0.8787 & 0.8792 & 0.8799\\
%LINE & 0.8969 & 0.9002 & 0.9010 & 0.9016 & 0.9017\\
%\midrule
%PTE & 0.9023 & 0.9061 & 0.9068 & 0.9077 & 0.9082\\
%Metapath2vec & 0.9319 & 0.9356 & 0.9365 & 0.9365 & 0.9369\\
%PMSW-metapath & 0.9440 & 0.9503 & 0.9513 & 0.9516 & 0.9519\\
%\midrule
%PMSW-metaschema & {\bf 0.9479} & {\bf 0.9617} & {\bf 0.9637} & {\bf 0.9640} & {\bf 0.9638}\\
%\bottomrule
%\end{tabular}
%% \vspace{-0.1in}
%\end{table}


%\begin{table}[!htb]
%\caption{\label{Tab:classify-author-DBIS}Experimental results of author node classification on the DBIS dataset.}\small
%\vspace{-0.1in}
%\centering
%% \renewcommand\arraystretch{0.5}
%\begin{tabular}{ccccccccccc}
%\toprule
%Macro-F1 & 10\% & 30\% & 50\% & 70\% & 90\% \\
%\midrule
%DeepWalk & 0.3195 & 0.3823 & 0.3898 & 0.3992 & 0.3945\\
%Node2vec & 0.3245 & 0.3873 & 0.3938 & 0.4042 & 0.3995\\
%LINE & 0.3096 & 0.3765 & 0.3828 & 0.3934 & 0.3885\\
%\midrule
%PTE & 0.3080 & 0.3748 & 0.3810 & 0.3922 & 0.3872\\
%Metapath2vec & 0.4306 & 0.5116 & 0.5342 & 0.5476 & 0.5448\\
%PMSW-metapath & 0.5067 & 0.5561 & 0.5751 & 0.5775 & 0.5839\\
%\midrule
%PMSW-metaschema & {\bf 0.5294} & {\bf 0.5798} & {\bf 0.5909} & {\bf 0.5919} & {\bf 0.5956}\\
%\toprule
%Micro-F1 & 10\% & 30\% & 50\% & 70\% & 90\% \\
%\midrule
%DeepWalk & 0.3488 & 0.3953 & 0.4011 & 0.4069 & 0.4067 \\
%Node2vec & 0.3538 & 0.4003 & 0.4051 & 0.4119 & 0.4107\\
%LINE & 0.3430 & 0.3905 & 0.3951 & 0.3969 & 0.4009\\
%\midrule
%PTE & 0.3418 & 0.3894 & 0.3937 & 0.3950 & 0.3989\\
%Metapath2vec & 0.4866 & 0.5308 & 0.5459 & 0.5545 & 0.5535\\
%PMSW-metapath & 0.5331 & 0.5619 & 0.5808 & 0.5838 & 0.5910\\
%\midrule
%PMSW-metaschema & {\bf 0.5538} & {\bf 0.5865} & {\bf 0.6043} & {\bf 0.6063} & {\bf 0.6096}\\
%\bottomrule
%\end{tabular}
%% \vspace{-0.05in}
%\end{table}


%\begin{table}[t]
%\caption{\label{Tab:classify-venue-AMiner}Experimental results of venue node classification on the AMiner dataset.}\small
%\vspace{-0.1in}
%\centering
%% \renewcommand\arraystretch{0.5}
%\begin{tabular}{ccccccccccc}
%\toprule
%Macro-F1 & 10\% & 30\% & 50\% & 70\% & 90\% \\
%\midrule
%DeepWalk & 0.3796 & 0.6695 & 0.7812 & 0.8674 & 0.8357\\
%Node2vec & 0.4486 & 0.7767 & 0.8394 & 0.8935 & 0.9177\\
%LINE & 0.4629 & 0.8473 & 0.9203 & 0.9466 & 0.9466\\
%\midrule
%PTE & 0.3388 & 0.8304 & 0.9210 & 0.9505 & 0.9489\\
%Metapath2vec & 0.5247 & 0.8971 & 0.9532 & 0.9701 & 0.9670\\
%PMSW-metapath & 0.5844 & 0.9403 & 0.9772 & 0.9786 & 0.9711\\
%\midrule
%PMSW-metaschema & {\bf 0.6056} & {\bf 0.9591} & {\bf 0.9774} & {\bf 0.9800} & {\bf 0.9789}\\
%\toprule
%Micro-F1 & 10\% & 30\% & 50\% & 70\% & 90\% \\
%\midrule
%DeepWalk & 0.4042 & 0.7166 & 0.7990 & 0.8877 & 0.9186 \\
%Node2vec & 0.4981 & 0.7957 & 0.8586 & 0.9145 & 0.9451\\
%LINE & 0.5167 & 0.8457 & 0.9209 & 0.9500 & 0.9571\\
%\midrule
%PTE & 0.4267 & 0.8372 & 0.9239 & 0.9550 & 0.9571\\
%Metapath2vec & 0.5975 & 0.9011 & 0.9522 & 0.9725 & 0.9857\\
%PMSW-metapath & 0.6309 & 0.9675 & 0.9704 & 0.9724 & 0.9772\\
%\midrule
%PMSW-metaschema & {\bf 0.6721} & {\bf 0.9723} & {\bf 0.9806} & {\bf 0.9838} & {\bf 0.9890}\\
%\bottomrule
%\end{tabular}
%% \vspace{-0.1in}
%\end{table} 
% For AMiner dataset, we follow~\cite{YuxiaoDong2017} to match the eight categories\footnote{The eight categories are: Computational Linguistics, Computer Graphics, Computer Networks and Wireless Communication, Computer Vision and Pattern Recognition, Computing Systems, Databases and Information Systems, Human Computer Interaction, Theoretical Computer Science.} of venues in Google Scholar\footnote{\url{https://scholar.google.com/citations?view_op=top_venues\&hl=en\&vq=eng}} with those in AMiner data, and get 133 labeled venues and $246,678$ labeled authors.
% Then, We employ the eight-category author and venue nodes to evaluate the performances of classification task and clustering task.

% Note that the node representations are learned from the full
% dataset. The embeddings of above labeled nodes are then used as
% the input to a logistic regression classifier and a $k$-means cluster. 
% In the classification experiments, we vary the size of the training set from 10\% to 90\% and the remaining nodes for testing. 
% We repeat each prediction experiment ten times and report the average performance in terms of both Macro-F1 and Micro-F1 scores.
% In the clustering experiments, we evaluate the clustering results in terms of normalized mutual information (NMI), and also, all the clustering experiments are conducted ten times and the average performance is reported.

%\subsection{Results and Analysis}
%In this section, we evaluate the embeddings learned by different models in terms of the node classification performance and the node clustering performance on the AMiner dataset and the DBIS dataset.





\begin{table*}[!htb]
 	\small
%	\footnotesize
	\caption{\small The Micro-F1 scores for multi-label node classification. ``--'' indicates that the used meta-path/meta-graph cannot generate embeddings for nodes of target type.}\label{Tab:classify_results}
	\vspace{-0.15in}
	\centering
	 \renewcommand\arraystretch{0.9}
	\begin{tabular}{p{2.8cm}<{\centering}|p{0.9cm}<{\centering}|p{0.9cm}<{\centering}|p{0.9cm}<{\centering}|p{0.9cm}<{\centering}|p{0.9cm}<{\centering}|p{0.9cm}<{\centering}|p{0.9cm}<{\centering}|p{0.9cm}<{\centering}|p{0.9cm}<{\centering}|p{0.9cm}<{\centering}|p{0.9cm}<{\centering}}
		\toprule
		Dataset & \multicolumn{3}{c|}{ACM} & \multicolumn{2}{c|}{DBLP} & \multicolumn{4}{c|}{Douban} & \multicolumn{2}{c}{Yelp} \\
		\midrule
		Node Type & Paper & Author & Venue & Paper & Author & User & Movie & Director & Actor & User & Business \\
		\midrule
%		\hline
%		Metric & Micro-F1 (\%) & Macro-F1 (\%) & Micro-F1 (\%) & Macro-F1 (\%) \\
%		Metric & Micro-F1 & Macro-F1 & Micro-F1 & Macro-F1  \\
%		\midrule
%		\hline
%\multirow{12}{10cm}{Micro-F1} % {Micro-F1 \\ \ \ \ \ \ (\%)}
		DeepWalk &  
0.5746 & 0.5560 & 0.8198 & 0.6590 & 0.9231 & 0.7205 & 0.5606 & 0.6370 & 0.6592 & 0.5457 & 0.3393 \\
LINE &
0.5608 & 0.5887 & 0.8169 & 0.7120 & 0.9379 & 0.7431 & 0.5621 & 0.6396 & 0.6511 & 0.5324 & 0.3467 \\ 
PTE &
0.5613 & 0.5903 & 0.6838 & 0.6680 & 0.9368 & 0.7077 & 0.5595 & 0.5674 & 0.6260 & 0.5178 & 0.3360 \\
\midrule
Metapath2vec-$\mathcal P_{1}$ & 
0.5774 & 0.6004 & 0.7826 & 0.8220 & 0.9397 & 0.7681 & 0.5678 & -- & 0.6661 & 0.5585 & 0.3435 \\
Metapath2vec-$\mathcal P_{2}$ & 
0.5791 & 0.6164 & -- & 0.5920 & 0.8627 & 0.7622 & 0.5454 & 0.6225 & -- & 0.5648 & 0.2864 \\ 
%\cline{1-12}
\hline
Metagraph2vec-$\mathcal S_{1}$ & 
0.5688 & 0.6122 & 0.7880 & 0.8273 & 0.9365 & 0.7924 & 0.5842 & 0.6509 & 0.6669 & 0.6045 & 0.3529 \\ 
Metagraph2vec-$\mathcal S_{2}$ & 
0.6108 & 0.6486 & 0.7990 & 0.8076 & 0.9506 & 0.7953 & 0.5535 & 0.6115 & 0.6366 & 0.6012 & 0.3482 \\ 
\midrule
SpaceyMetapath-$\mathcal P_{1}$ &
0.5805 & 0.6140 & 0.8185 & 0.8410 & 0.9439 & 0.7864 & 0.5711 & -- & 0.6839 & 0.6006 & 0.3574 \\
SpaceyMetapath-$\mathcal P_{2}$ & 
0.5880 & 0.6413 & -- & 0.6300 & 0.8836 & 0.7768 & 0.5596 & 0.6368 & -- & 0.5870 & 0.3312 \\
\hline
SpaceyMetagraph-$\mathcal S_{1}$ & 
0.5750 & 0.6171 & 0.8094 & {\bf 0.8520} & 0.9438 & {\bf 0.8036} & {\bf 0.5889} & {\bf 0.6676} & {\bf 0.6906} & {\bf 0.6101} & {\bf 0.3627} \\
SpaceyMetagraph-$\mathcal S_{2}$ & 
0.6136 & {\bf 0.6574} & {\bf 0.8412} & 0.8410 & {\bf 0.9521} & 0.8017 & 0.5720 & 0.6522 & 0.6809 & 0.6072 & 0.3524 \\ 
\hline
SpaceyMetaschema & 
{\bf 0.6145} & 0.6493 & 0.8369 & 0.8330 & 0.9512 & 0.8032 & 0.5793 & 0.6535 & 0.6832 & 0.5688 & 0.3536 \\ 
		\bottomrule
	\end{tabular}
	 \vspace{-0.05in}
\end{table*}


\begin{table*}[!htb]
	\small
	%		\footnotesize
	\caption{\small The Macro-F1 scores  for multi-label node classification. ``--'' indicates that the used meta-path/meta-graph cannot generate embeddings for nodes of target type.}\label{Tab:classify_results_macro}
	\vspace{-0.15in}
	\centering
	\renewcommand\arraystretch{0.9}
	\begin{tabular}{p{2.8cm}<{\centering}|p{0.9cm}<{\centering}|p{0.9cm}<{\centering}|p{0.9cm}<{\centering}|p{0.9cm}<{\centering}|p{0.9cm}<{\centering}|p{0.9cm}<{\centering}|p{0.9cm}<{\centering}|p{0.9cm}<{\centering}|p{0.9cm}<{\centering}|p{0.9cm}<{\centering}|p{0.9cm}<{\centering}}
		\toprule
		Dataset & \multicolumn{3}{c|}{ACM} & \multicolumn{2}{c|}{DBLP} & \multicolumn{4}{c|}{Douban} & \multicolumn{2}{c}{Yelp} \\
		\midrule
		Node Type & Paper & Author & Venue & Paper & Author & User & Movie & Director & Actor & User & Business \\
		\midrule
		% 		%		\hline
		% 		%		Metric & Micro-F1 (\%) & Macro-F1 (\%) & Micro-F1 (\%) & Macro-F1 (\%) \\
		% 		%		Metric & Micro-F1 & Macro-F1 & Micro-F1 & Macro-F1  \\
		% 		%		\midrule
		% 		%		\hline
		% 		\multirow{12}{10cm}{Micro-F1} % {Micro-F1 \\ \ \ \ \ \ (\%)}
		% 		& DeepWalk &  
		% 		0.5746 & 0.5560 & 0.8198 & 0.6590 & 0.9231 & 0.7205 & 0.5606 & 0.6370 & 0.6592 & 0.5457 & 0.3393 \\
		% 		& LINE &
		% 		0.5608 & 0.5887 & 0.8169 & 0.7120 & 0.9379 & 0.7431 & 0.5621 & 0.6396 & 0.6511 & 0.5324 & 0.3467 \\ 
		% 		& PTE &
		% 		0.5613 & 0.5903 & 0.6838 & 0.6680 & 0.9368 & 0.7077 & 0.5595 & 0.5674 & 0.6260 & 0.5178 & 0.3360 \\
		% 		& Metapath2vec-$\mathcal P_{1}$ & 
		% 		0.5774 & 0.6004 & 0.7826 & 0.8220 & 0.9397 & 0.7681 & 0.5678 & -- & 0.6661 & 0.5585 & 0.3435 \\
		% 		& Metapath2vec-$\mathcal P_{2}$ & 
		% 		0.5791 & 0.6164 & -- & 0.5920 & 0.8627 & 0.7622 & 0.5454 & 0.6225 & -- & 0.5648 & 0.2864 \\ 
		% 		& Metagraph2vec-$\mathcal S_{1}$ & 
		% 		0.5688 & 0.6122 & 0.7880 & 0.8273 & 0.9365 & 0.7924 & 0.5842 & 0.6509 & 0.6669 & 0.6045 & 0.3529 \\ 
		% 		& Metagraph2vec-$\mathcal S_{2}$ & 
		% 		0.6108 & 0.6486 & 0.7990 & 0.8076 & 0.9506 & 0.7953 & 0.5535 & 0.6115 & 0.6366 & 0.6012 & 0.3482 \\ 
		% 		& SpaceyMetapath-$\mathcal P_{1}$ &
		% 		0.5805 & 0.6140 & 0.8185 & 0.8410 & 0.9439 & 0.7864 & 0.5711 & -- & 0.6839 & 0.6006 & 0.3574 \\
		% 		& SpaceyMetapath-$\mathcal P_{2}$ & 
		% 		0.5880 & 0.6413 & -- & 0.6300 & 0.8836 & 0.7768 & 0.5596 & 0.6368 & -- & 0.5870 & 0.3312 \\
		% 		& SpaceyMetagraph-$\mathcal S_{1}$ & 
		% 		0.5750 & 0.6171 & 0.8094 & {\bf 0.8520} & 0.9438 & {\bf 0.8036} & {\bf 0.5889} & {\bf 0.6676} & {\bf 0.6906} & {\bf 0.6101} & {\bf 0.3627} \\
		% 		& SpaceyMetagraph-$\mathcal S_{2}$ & 
		% 		0.6136 & {\bf 0.6574} & {\bf 0.8412} & 0.8410 & {\bf 0.9521} & 0.8017 & 0.5720 & 0.6522 & 0.6809 & 0.6072 & 0.3524 \\ 
		% 		& SpaceyMetaschema & 
		% 		{\bf 0.6145} & 0.6493 & 0.8369 & 0.8330 & 0.9512 & 0.8032 & 0.5793 & 0.6535 & 0.6832 & 0.5688 & 0.3536 \\ 
		% 		\bottomrule
		
		DeepWalk & 
		0.1983 & 0.2403 & 0.3705 & 0.6504 & 0.9175 & 0.1789 & 0.3136 & 0.2408 & 0.2661 & 0.0584 & 0.1187 \\
		LINE & 
		0.1891 & 0.2358 & 0.3649 & 0.6863 & 0.9238 & 0.2064 & 0.3120 & 0.2221 & 0.2382 & 0.0389 & 0.1164 \\
		PTE &
		0.1941 & 0.2474 & 0.3780 & 0.6376 & 0.9218 & 0.1687 & 0.2962 & 0.2279 & 0.2405 & 0.0314 & 0.1065 \\
		\midrule
		Metapath2vec-$\mathcal P_{1}$ & 
		0.1682 & 0.2408 & 0.4239 & 0.8073 & 0.9344 & 0.3703 & 0.2871 & -- & 0.2732 & 0.0683 & 0.1147 \\
		Metapath2vec-$\mathcal P_{2}$ & 
		0.2019 & 0.3174 & -- & 0.5110 & 0.8605 & 0.3288 & 0.2537 & 0.2305 & -- & 0.0782 & 0.0609 \\ 
		\hline	
		Metagraph2vec-$\mathcal S_{1}$ &
		0.1757 & 0.2973 & 0.4398 & 0.7988 & 0.9309 & 0.3958 & 0.3117 & 0.2571 & 0.2767 & 0.1362 & 0.1337 \\ 
		Metagraph2vec-$\mathcal S_{2}$ &
		0.2113 & 0.3080 & 0.4254 & 0.7832 & 0.9462 & 0.3866 & 0.2606 & 0.2176 & 0.2351 & 0.1217 & 0.1263 \\ 
		\midrule
		SpaceyMetapath-$\mathcal P_{1}$ &
		0.1797 & 0.2817 & 0.4518 & 0.8329 & 0.9399 & 0.3827 & 0.2921 & -- & 0.3101 & 0.1297 & 0.1310 \\ 
		SpaceyMetapath-$\mathcal P_{2}$ & 
		0.2123 & 0.3571 & -- & 0.5506 & 0.8774 & 0.3613 & 0.2767 & 0.2615 & -- & 0.0968 & 0.1089 \\ 
		\hline
		SpaceyMetagraph-$\mathcal S_{1}$ & 
		0.1862 & 0.3290 & 0.4616 & {\bf 0.8361} & 0.9363 & {\bf  0.4131} & {\bf 0.3154} & {\bf 0.2859} & {\bf 0.3247} & {\bf 0.1476} & {\bf 0.1431} \\ 
		SpaceyMetagraph-$\mathcal S_{2}$ & 
		0.2188 & 0.3511 & 0.4629 & 0.8243 & {\bf 0.9485} & 0.4015 & 0.2890 & 0.2678 & 0.3030 & 0.1270 & 0.1315 \\ 
		\hline
		SpaceyMetaschema &
		{\bf 0.2304} & {\bf 0.3587} & {\bf 0.4641} & 0.8196 & 0.9478 & 0.3827 & 0.3012 & 0.2699 & 0.3120 & 0.0768 & 0.1268 \\ 
		\bottomrule
	\end{tabular}
	\vspace{-0.1in}
\end{table*}



%\vspace{-0.15in}
\subsection{Multi-label Node Classification}
%For each dataset, we first learn the node embedding vectors from the full dataset, and then use the embeddings of the labeled nodes (as introduced in Section~\ref{sec:dataset}) as the input to a logistic regression classifier.
%We use different ratios of the data (from 10\% to 90\%) for training and the others for testing, and use Micro-F1 score and Macro-F1 score as metrics for evaluation.
%The experimental results are shown in Table~\ref{Tab:classify-author-AMiner}, Table~\ref{Tab:classify-author-DBIS}, and Table~\ref{Tab:classify-venue-AMiner} (since there are too few venues to be classified in the DBIS dataset, we only test author classification on this dataset).
%
%By varying the train-test split ratio, we can observe that the proposed \textit{PMSW-metapath} and \textit{PMSW-metaschema} consistently outperform all baselines in terms of both metrics.
%For the author node classification, \textit{PMSW-metapath} and \textit{PMSW-metaschema} improve the classification performance in different train-test ratios by 6\%-23\% over DeepWalk, LINE, and Node2vec, and by 1\%-23\% over PTE and Metapath2vec, respectively.
%For the venue node classification, the improvement is consistent, on average by 1\%-28\% over baseline models.
%Especially,
%we can see that \textit{PMSW-metapath} and \textit{PMSW-metaschema} are quite robust and can achieve big gains when given a small size of training data. 
%% For example, given 10\% of nodes as training data, \textit{PMSW-metapath} and \textit{PMSW-metaschema} achieve 16\%-50\% improvements in terms of Macro-
%% F1 and 8\%-47\% gains in terms of Micro-F1 over DeepWalk / node2vec, LINE, and PTE.
%In addition, we find that \textit{PMSW-metaschema} can achieve on average 1\% improvement compared with \textit{PMSW-metapath},
%which indicates that an ensemble of multiple meta-paths is more effective than a single meta-path, which may capture an ensemble of semantic and structural correlations.
%Due to the lack of space, we sample one datasets (50\% training for author node classification) and present the p-values in t-test results in Table~\ref{Tab:significant-test}.
%The results prove the effectiveness of the proposed two frameworks.


For the node classification task, %we use all datasets (as introduced in Section~\ref{sec:dataset}), where a node can be assigned one or more labels.
%For each dataset, 
we first learn the node embedding vectors from the full nodes on each dataset, and then use the embeddings of the labeled nodes as input features for a one-vs-rest logistic regression classifier. %where the  train-test-split is 1:1.
We repeat each classification experiment ten times by randomly splitting 50\% of the labeled nodes for training and the others for testing, and report the average performance in terms of both Micro-F1 score and Macro-F1 score.
We also calculate the variances of the scores to reflect the significance of the experimental results.
% Due to the lack of space, the Micro/Macro-F1 scores are shown in Table~\ref{Tab:classify_results} and Table~\ref{Tab:classify_results_macro}, and their variances are shown in the supplementary material. $\blacksquare$


We can observe that our proposed algorithms consistently outperform all the start-of-the-art baselines in both metrics on all datasets.
For example, 
%on the ACM dataset, we improve the classification performance in different node types by 0.03--0.11 (relatively 16\%--31\%) over DeepWalk, LINE and PTE, and 0.02--0.09 (relatively 10\%--36\%) over Metapath2vec and Metagraph2vec, in terms of Macro-F1 scores.
%In other three datasets, the improvements are consistent.
for the author node classification on the ACM dataset,
our proposed models outperform all baseline models by around 0.01--0.10 (relatively 1\%--18\%) in terms of Micro-F1 scores and by around 0.04--0.12 (relatively 13\%--52\%) in terms of Macro-F1 scores.
% For other classification cases, the effects are consistent.
% Specially, 
% it is evident we can see how the proposed spacey random walk strategy in exploring heterogeneous neighborhoods performs much better than 
% %the other benchmark algorithms.
% %Compared with 
% the normal meta-path/meta-graph based random walk sampling algorithms (e.g., Metapath2vec and Metagraph2vec).
% %For the case of author node classification on the ACM dataset, 
Moreover, given the same meta-path or meta-graph, the proposed {\it SpaceyMetapath}/{\it SpaceyMetagraph} imporves the author node classification performance by around 0.01--0.03 in Micro-F1 score and 0.03--0.04 in Macro-F1 score over Metapath2vec/Metagraph2vec.
%For other cases, the effectiveness can be similarly observed, for example, 
% Similarly, we can consistently observe the effectiveness of deploying spacey random walk in other cases,
% for example, compared with Metapath2vec/Metagraph2vec, we can find {\it SpaceyMetapath}/{\it SpaceyMetagraph} achieves the gains of 
% %0.02--0.04 in both Micro-F1 score and Macro-F1 score for the venue node classification on ACM,
% 0.02--0.04 in Micro-F1 and 0.03--0.04 in Macro-F1 for the paper node classification on DBLP,
% %0.01--0.02 in Micro-F1 and 0.01--0.04 in Macro-F1 for the user node classification on Douban,
% 0.01--0.05 in Micro-F1 and 0.01--0.04 in Macro-F1 for the business node classification on Yelp,
% etc.

In most cases, we can find that,
by capturing the semantically meaningful information of an appropriate meta-path or meta-graph,
the meta-path/meta-graph driven algorithms (including our proposed methods and Metapath2vec and Metagraph2vec) obviously outperform DeepWalk, LINE and PTE.
Among them, meta-graph driven algorithms can achieve better performance than meta-path driven algorithms by capturing richer semantics of integrating multiple meta-paths. 
In addition, % it is worth mentioning that
we can find that
the proposed {\it SpaceyMetaschema} achieves competitive performance compared with the best of other methods,
which may be more practical in complex networks with a large variety of types for the dispense with handcrafted domain-specific meta-paths/meta-graphs.



%\begin{table}[t]
%\caption{\label{Tab:significant-test}P-value for significance test for author node classification (50\% training data) and clustering on AMiner dataset.}\small
%\vspace{-0.1in}
%\centering
%% \renewcommand\arraystretch{0.5}
%\begin{tabular}{cccc}
%\toprule
%Classification & Metapath2vec & PMSW- & PMSW-\\
% &  & metapath & metaschema\\
%\midrule
%Metapath2vec & -- & 7.010e-12 & 2.588e-05 \\
%PMSW-metapath & -- & -- & 1.047e-02 \\
%PMSW-metaschema & -- & -- & -- \\
%\midrule
%Clustering & Metapath2vec & PMSW- & PMSW-\\
% &  & metapath & metaschema\\
%\midrule
%Metapath2vec & -- & 7.184e-03 & 1.641e-04 \\
%PMSW-metapath & -- & -- & 3.768e-03 \\
%PMSW-metaschema & -- & -- & -- \\
%\bottomrule
%\end{tabular}
%%\vspace{-0.1in}
%\end{table}




%\subsection{Node Clustering}
%%We also use the eight-category author and venue nodes in AMiner dataset to evaluate the performance of the representations learned by embedding methods on the node clustering task.
%%We use the $k$-means algorithm to cluster the data and evaluate the clustering results with metric normalized mutual information (NMI).
%%Table~\ref{Tab:cluster-AMiner} shows the experimental results.
%In the clustering experiments, we also employ the ACM and DBLP datasets to compare different embedding methods.
%We use the the embeddings of the labeled nodes as the input to a  $k$-means cluster and evaluate the clustering results  in terms of NMI (Normalized Mutual Information) score, 
%and also, all the clustering experiments are conducted ten times and the average performance is reported.
%The experimental results are shown in Table XXX.






%\begin{table}[t]
%\caption{\label{Tab:cluster-AMiner}Experimental results of node clustering on the AMiner dataset.}\small
%%\vspace{-0.15in}
%\centering
%% \renewcommand\arraystretch{0.5}
%\begin{tabular}{cccc}
%\toprule
%NMI & author & venue\\
%\midrule
%DeepWalk & 0.4941 & 0.8521 \\
%Node2vec & 0.6246 & 0.8902 \\
%LINE & 0.6423 & 0.8967 \\
%\midrule
%PTE & 0.6483 & 0.9060 \\
%metapath2vec & 0.7470 & 0.9274 \\
%PMSW-metapath & 0.7685 & 0.9306 \\
%\midrule
%PMSW-metaschema & {\bf 0.7794} & {\bf 0.9356} \\
%\bottomrule
%\end{tabular}
%%\vspace{-0.1in}
%\end{table}


%Overall, the results of node clustering are consistent with the results of node classification.
%And we can reach a similar conclusion as analyzed in node classification experiments.
%% we can consistently conclude the efficacy and stability of proposed methods as analyzed in section 4.3.
%We can see that \textit{PMSW-metapath} and \textit{PMSW-metaschema} outperform all the comparative methods.
%When clustering for authors, \textit{PMSW-metapath} and \textit{PMSW-metaschema} achieve 12\%-28\% improvements over DeepWalk, LINE, and Node2vec, and 2\%-13\% gains over PTE and Metapath2vec.
%When clustering for venues, they achieve high NMI scores and outperform base methods by 1\%-8\%. 
%We also present the p-values in t-test results for author node clustering in Table~\ref{Tab:significant-test}.
%
%
%In summary, the proposed \textit{PMSW-metapath} and \textit{PMSW-metaschema} can effectively deal with the network heterogeneity challenge--the diversity of multiple types of nodes and their relationships, and thus learn much better semantically meaningful node representations on the heterogeneous networks.


\begin{table}[!htb]
	\small
	%		\footnotesize
	\caption{\small Binary operators for learning edge features. The definitions correspond to the $i$-th component of vector ${\mathbf u}$ and ${\mathbf v}$.}\label{Tab:binary_operators}
	\vspace{-0.15in}
	\centering
	\renewcommand\arraystretch{0.7}
	\begin{tabular}{c|c|c|c|c}
		\toprule
		Operator & Average & Hadamard & Weighted-L1 & Weighted-L2 \\
		\midrule
		Definition & $({\mathbf u}_i+{\mathbf v}_i) / 2$ & ${\mathbf u}_i * {\mathbf v}_i$ & $|{\mathbf u}_i - {\mathbf v}_i|$ & ${|{\mathbf u}_i - {\mathbf v}_i|}^2$ \\
		\bottomrule
	\end{tabular}
	\vspace{-0.15in}
\end{table}



\begin{table*}[t]
	 	\small
%		\footnotesize
	\caption{\small The mean AUC scores for link prediction. ``--'' indicates that the used meta-path/meta-graph cannot generate embeddings for nodes of target type. The edge types for each dataset are shown in Figure~\ref{Fig:datasets}.}\label{Tab:lp_results}
	\vspace{-0.15in}
	\centering 
	\renewcommand\arraystretch{0.9}
	\begin{tabular}{p{2.8cm}<{\centering}|p{0.8cm}<{\centering}|p{0.8cm}<{\centering}|p{0.8cm}<{\centering}|p{0.8cm}<{\centering}|p{0.8cm}<{\centering}|p{0.8cm}<{\centering}|p{0.8cm}<{\centering}|p{0.8cm}<{\centering}|p{0.8cm}<{\centering}|p{0.8cm}<{\centering}|p{0.8cm}<{\centering}|p{0.8cm}<{\centering}}
		\toprule
		Dataset & \multicolumn{3}{c|}{ACM} & \multicolumn{3}{c|}{DBLP} & \multicolumn{3}{c|}{Douban} & \multicolumn{3}{c}{Yelp} \\
		\midrule
		Edge Type & P--P & P--V & P--T & P--A & P--C & P--T & U--U & U--M & M--D & U--U & U--B & B--C \\
		\midrule
		DeepWalk &
		0.8711 & 0.8775 & 0.6640 & 0.8743 & 0.9219 & 0.8777 & 0.6255 & 0.7906 & 0.8397 & 0.8768 & 0.8815 & 0.9212 \\ 
		LINE &
		0.8555 & 0.8550 & 0.6454 & 0.8180 & 0.8550 & 0.7479 & 0.6374 & 0.7850 & 0.8069 & 0.8770 & 0.8545 & 0.9063 \\ 
		PTE &
		0.6734 & 0.7189 & 0.5776 & 0.6410 & 0.7189 & 0.5901 & 0.6691 & 0.6461 & 0.5881 & 0.8319 & 0.7969 & 0.8244 \\\midrule
		Metapath2vec-$\mathcal P_{1}$ &
		0.7137 & 0.9486 & -- & 0.8801 & 0.9532 & -- & 0.6061 & 0.7994 & -- & 0.6464 & 0.8382 & 0.9179 \\
		Metapath2vec-$\mathcal P_{2}$ &
		0.7392 & -- & 0.7307 & 0.8848 & -- & 0.8900 & 0.6006 & 0.8099 & 0.8793 & 0.7333 & 0.7841 & -- \\\hline
		Metagraph2vec-$\mathcal S_{1}$ &
		0.7257 & 0.9393 & -- & 0.8887 & 0.9438 & -- & 0.6097 & 0.8081 & 0.8907 & 0.6493 & 0.8664 & 0.9081 \\ 
		Metagraph2vec-$\mathcal S_{2}$ &
		0.7313 & 0.9467 & 0.6865 & 0.8925 & 0.9555 & 0.8765 & 0.6728 & 0.7711 & 0.8624 & 0.6919 & 0.8718 & -- \\\midrule
		SpaceyMetapath-$\mathcal P_{1}$ &
		0.7236 & 0.9521 & -- & 0.8901 & 0.9596 & -- & 0.6206 & 0.8318 & -- & 0.6668 & 0.8565 & 0.9371 \\
		SpaceyMetapath-$\mathcal P_{2}$ &
		0.7432 & -- & {\bf 0.7365} & 0.8870 & -- & {\bf 0.8926} & 0.6152 & 0.8310 & 0.8976 & 0.7507 & 0.8516 & -- \\\hline
		SpaceyMetagraph-$\mathcal S_{1}$ &
		0.7292 & 0.9427 & -- & 0.8911 & 0.9511 & -- & 0.6240 & 0.8339 & {\bf 0.9022} & 0.6537 & 0.8848 & 0.9242 \\
		SpaceyMetagraph-$\mathcal S_{2}$ &
		0.7333 & {\bf 0.9523} & 0.6889 & {\bf 0.8956} & 0.9618 & 0.8830 & 0.6903 & 0.8011 & 0.9009 & 0.6976 & 0.8868 & -- \\\hline
		SpaceyMetaschema &
		{\bf 0.9238} & 0.9385 & 0.6731 & 0.8867 & {\bf 0.9655} & 0.8824 & {\bf 0.9338} & {\bf 0.8734} & 0.9015 & {\bf 0.9254} & {\bf 0.8970} & {\bf 0.9497} \\
		\bottomrule
	\end{tabular}
	\vspace{-0.1in}
\end{table*}






\subsection{Link Prediction}
%For the link prediction task, 
%we test the performance of different embedding methods on the Douban and Yelp datasets.
For each dataset, 
we follow \cite{GroverL16} to randomly hide 20\% of edges of each edge type as missing edges.
Then, we learn the embedding using the rest of the 80\% edges and predict these missing edges.
%For the prediction model, we generate the labeled dataset of edges as follows:
%For the computational effciency, we randomly sample 2,048 edges (from the 80\% training edges) as positive examples, and equally split them into two partitions $E_{train}$ and $E_{test}$.
%To generate negative examples, we randomly sample 2,048 edges  (from the 20\% missing edges) and equally split them into two partitions $E_{train}^-$ and $E_{test}^-$.
For the computational effciency, we randomly sample 2,048 edges (from the 20\% hided edges) as positive examples and equally split them into two partitions $E_{train}$ and $E_{test}$.
We also randomly sample 2,048 unobserved edges as negative examples and equally split them into two partitions $E_{train}^-$ and $E_{test}^-$.
Then, we consider the link prediction evaluation as a binary classification problem with  $(E_{train}, E_{train}^-)$ for training and  $(E_{test}, E_{test}^-)$ for testing.
We study several binary operators~\cite{GroverL16} (as shown in Table~\ref{Tab:binary_operators}) to construct features for an edge based on its two node vectors, and then the operated feature vector for an edge is as the input to a logistic regression classifier.
We repeat the above link prediction experiment ten times and report the average performance in terms of AUC (Area Under Curve) score.
%The experimental results are shown in Table~\ref{Tab:lp_results_Douban} and Table~\ref{Tab:lp_results_Yelp}.
% Due to the lack of space, we show the mean value of four AUC scores (one for each binary operator) in Table~\ref{Tab:lp_results} and separately show them in the supplementary material. $\blacksquare$ 


%We can see that the proposed {\it SpaceyMetapath}, {\it SpaceyMetagraph}, and {\it SpaceyMetaschema} outperform all the comparative methods on all datasets.
%%On the Douban dataset, the proposed methods consistently improve the link prediction performance of different evaluated edge types by around 0.02--0.16 (relatively 2\%--19\%) over DeepWalk, LINE and PTE, and around 0.01--0.36 (relatively 1\%--57\%) over Metapath2vec and Metagraph2vec, in terms of the AUC scores for the best possible choices of the binary operator for each algorithm.
%%On the Yelp dataset, the improvements are consistent, and we can observe that the proposed methods achieve 0.01--0.27 gains over all baseline methods in all the link prediction experiments of different edge types.
%For example, 
%for the {\it Paper}--{\it Paper} (P--P) link prediction on the ACM dataset,
%%on the ACM dataset, we improve the link prediction performance of different evaluated edge types by around 
%the proposed methods improve the mean AUC scores by around
%0.05--0.25 (relatively 6\%--37\%) over DeepWalk, LINE and PTE,
%and 0.18--0.21 (relatively 25\%--29\%) over Metapath2vec and Metagraph2vec.
%%in terms of the mean AUC scores.
%%In more detail, 
%For the {\it User}--{\it User} (U--U) link prediction on the Yelp dataset,
%the proposed methods achieve around 0.06--0.07 (relatively 7\%--8\%) over DeepWalk, LINE and PTE,
%and around 0.17--0.27 (relatively 22\%--40\%) over Metapath2vec and Metagraph2vec, for the best possible choices of the binary operator for each algorithm.


Overall, the results of link prediction are consistent with the results of node classification, and we can reach a similar conclusion as analyzed in node classification experiment.
We can see that the proposed methods clearly achieve better performance than the comparative methods on all datasets.
For example, 
on the ACM dataset,
we improve the link prediction performance of different edge types by around 0.05--0.25 (relatively 6\%--37\%) over DeepWalk, LINE and PTE, and 0.01--0.21 (relatively 1\%--29\%) over Metapath2vec and Metagraph2vec, in terms of the mean AUC score.
For the detailed AUC scores of all binary operators (which are reported in the supplementary material), the improvements are consistent.
For example, on the DBLP dataset,
we can observe that the proposed methods achieve 0.01--0.09 (relatively 1\%--10\%) gains over all baseline methods in all the link prediction experiments of different edge types, in terms of the best possible choice of the binary operators for each algorithm.
Moreover,
we can also evidently observe the effectiveness of the proposed spacey random walk compared with the normal meta-path/meta-graph based random walk.
In most cases, given the same meta-path or meta-graph, the proposed {\it SpaceyMetapath}/{\it SpaceyMetagraph} can achieve around 0.01--0.07 improvements over Metapath2vec/Metagraph2vec in the link prediction experiments of different edge types on different datasets.


It is worth mentioning that, in some cases,
the {\it SpaceyMetaschema} significantly outperforms {\it SpaceyMetapath}/{\it SpaceyMetagraph}, e.g., for the P–P link prediction on the ACM dataset and the U-U link prediction on the Yelp dataset, the improvements are almost 0.2.
And even, in these cases, the homogeneous methods (e.g., DeepWalk and LINE ) can also perform better than the meta-path/meta-graph based methods.
The possible reason we believe is the specialities of the relations and the biases of the used meta-paths/meta-graphs.
A given meta-path/meta-graph usually expresses some important semantics, but may not be very sufficient to reflect other special link structures.
As a result, the methods which homogeneously cover all links (i.e., DeepWalk and LINE) and which dynamically treat all links with a superior spacey stragety (i.e.,  {\it SpaceyMetaschema}) abnormally achieve better performance in these cases.





%\subsection{Visualization}
%In this section, we visualize the embedding vectors for an intuitive understanding.
%Here we use the DBLP dataset and feed the embedding vectors of the labeled venue nodes  into the standard visualization tool t-SNE~\cite{maaten2008visualizing}.
%As a result, each venue is mapped as a 2-dimensional vector.
%Then, we visualize the 2-dimensional vector of each venue  as a point on a 2-dimensional space, and use different colors to indicate different labels.
%The visualization figures of different embedding methods are shown in Figure XXX.
%Note that for each embedding method, we use the 





\begin{figure*}[t]
%	\vspace{-0.1in}
	\small
	\setlength{\abovecaptionskip}{-0.1cm}
	\setlength{\belowcaptionskip}{-0.4cm}
	\centering
	\subfigure[\small walk-times $w$.]{
		\label{Fig:walk_times_P1}
		\includegraphics[width=0.3\textwidth]{resources/wt_acm_P1_classify_1_train_ratio_0_5_micro}
	}
	%     \hfill
	%	\hspace{0.1in}
	%    \vspace{0.0in}
	\subfigure[\small walk-length $l$.]{
		\label{Fig:walk_length_P1}
		\includegraphics[width=0.3\textwidth]{resources/wl_acm_P1_classify_1_train_ratio_0_5_micro}
	}
	%	\hspace{-0.1in}
	%    \vspace{0.in}
	\subfigure[\small personalized-probability $\alpha$.]
	{\label{Fig:personalized_probability_P1}
		\includegraphics[width=0.3\textwidth]{resources/alpha_acm_P1_classify_1_train_ratio_0_5_micro}
	}
	%     \hfill
	%	\hspace{0.1in}
	%    \vspace{0.in}
	%	\subfigure[\small scalability analysis.]
	%	{\label{Fig:scalability_time}
	%		\includegraphics[width=0.235\textwidth]{resources/scalability_time}
	%	}
	% \includegraphics[width=0.4\textwidth]{walk-times-author}
	\caption{\small Parameter sensitivity for author node classification on the ACM dataset.}
	\label{Fig:Parameter_sensitivity}
	
\end{figure*}




\vspace{-0.1in}
\subsection{Parameter Sensitivity}
\label{sec:Parameter_Sensitivity}
% For the proposed methods, there exist several important parameters, such as walk-times $t$, walk-length $l$, %neighborhood size $k$, 
% and personalized probability $\alpha$ (see in Eq.~(\ref{Eq:spacey_out_law})).
%Their default values are shown in Sec.~\ref{sec:exp_settings}.
In this section, we illustrate the parameters sensitivity %to the \textit{PMSW-metapath} model 
by the Micro-F1 scores of author node classification experiments on the ACM dataset. % given different meta-paths or meta-graphs.
%As a comparison, we also test the effects of varying walk-times and walk-length in normal meta-path/meta-graph based random walk sampling algorithms algorithms (i.e., Metapath2vec and Metagraph2vec), given different meta-paths/meta-graphs.
% Specially,
% to intuitively demonstrate the efficiency and effectiveness of the proposed spacey random walk strategy,
% we also test the effects of varying walk-times and walk-length in normal meta-path/meta-graph based random walk sampling algorithms (i.e., Metapath2vec and Metagraph2vec).
For each experiment, we vary one parameter and fix the others as the default values (as shown in Sec.~\ref{sec:exp_settings}).
%For the meta-path/meta-graph %based frameworks (i.e. {\it SpaceyMetapath} and {\it SpaceyMetagraph}), 
%we use meta-path $\mathcal P_1$ and meta-graph $\mathcal S_1$ (as shown in Figure~\ref{Fig:ACM_dataset}) as an example.
%Specially,
%to intuitively demonstrate the efficiency and effectiveness of the proposed ``spacey'' strategy,
%we also test the effects of varying walk-times and walk-length in normal meta-path/meta-graph based random walk sampling algorithms algorithms (i.e., Metapath2vec and Metagraph2vec). % without using ``spacey'' strategy.
%and analyse the speedup to achieve equivalent performance by using the ``spacey'' strategy.
%The results are shown in Figure~\ref{Fig:walk_times}, Figure~\ref{Fig:walk_length}, and Figure~\ref{Fig:personalized_probability}.
%The results are shown in Figure~\ref{Fig:Parameter_sensitivity}.
%Due to the lack of space, 
% For better visualization,
% we show the results with meta-path $\mathcal P_1$ and meta-graph $\mathcal S_1$ (as shown in Figure~\ref{Fig:ACM_dataset}) in Figure~\ref{Fig:Parameter_sensitivity}, and show the results with meta-path $\mathcal P_2$ and meta-graph $\mathcal S_2$ in the supplementary material. $\blacksquare$ 
% The results are shown in Figure~\ref{Fig:Parameter_sensitivity}.


From Figure~\ref{Fig:walk_times_P1} and Figure~\ref{Fig:walk_length_P1}, we can see that walk-times $w$ and walk-length $l$ are positive to %the author node classification
performance for all random walk based algorithms, and the positivity gradually weakens with the parameter increasing.
From Figure~\ref{Fig:personalized_probability_P1}, we can see that the performance increases with the  personalized probability $\alpha$ increasing, and the tend will be weakened when $\alpha$ reaches around 0.7.
%To reach a balance of computational cost and efficacy, we choose $w$=1000 and $l$=100 as their optimal values.
Specially, from Figure~\ref{Fig:Parameter_sensitivity},  
we can clearly observe that the proposed {\it SpaceyMetapath}/{\it SpaceyMetagraph} outperforms Metapath2vec/Metagraph2vec given a relatively small $w$ or $l$.
% which demonstrates that the proposed spacey random walk can efficiently improve the walk quality compared with the normal Marovian random walk.
For example,
%we can find that,
given meta-path $\mathcal P_1$ as the input, we can find that the performance of the proposed {\it SpaceyMetapath} with $l\!=\!40$ is equivalent to the performance of Metapath2vec with $l\!=\!640$, giving us around 16x speedup.
% Also,
% given meta-path $\mathcal P_2$ as the input, {\it SpaceyMetapath} with $l\!=\!80$ achieves equivalent performance to Metapath2vec with $l\!=\!640$, giving us around 8x speedup.
%the performance of the proposed {\it SpaceyMetapath} with $l=80$ is equivalent to the performance of Metagraph2vec with with $l=500$, giving us more than 3x speedup.
Further,
we randomly trace 1000 walk sequences of meta-path $\mathcal P_1$ guided spacey random walk and normal Marovian random walk respectively,
and gradually compute the JS (Jensen--Shannon) divergence~\cite{fuglede2004jensen} of the node distributions between steps.
The average variation is shown in Figure~\ref{Fig:stationary_analysis_P1}.
Compared with Metapath2vec, 
we can evidently observe that the distribution divergence for {\it SpaceyMetapath} quickly descends to a small level with a small walk-length.
Overall, above comparision analysis indicates that the proposed spacey random walk frameworks are able to reach high performance under a cost-effective parameter choice (the smaller, the more efficient).
%by using the proposed spacey random walk,
%{\it SpaceyMetapath}, {\it SpaceyMetagraph}, and {\it SpaceyMetaschema} consistently and significantly outperform normal meta-path/meta-graph based random walk sampling algorithms (e.g., Metapath2vec and Metagraph2vec) given a small  walk-times and walk-length, especially using a meta-path as the constraint.


% This also demonstrates the positive effect of the proposed spacey random walk frameworks.
% And specially, it is worth mentioning that the normal meta-path/meta-graph based random walk algorithms (e.g., Metapath2vec and Metagraph2vec) can be seen as the special cases of our proposed frameworks when the personalized probability $\alpha=0$.
%the Micro-F1 score reaches its optimum value when $\alpha$=0.01, while it becomes lower with a larger or smaller value of $\alpha$.
%Similarly, Figure~\ref{Fig:window-size} suggests that window size $k$=8 is a proper choice, because with a bigger $k$, the result has a very weak increase in terms of clustering, and even has a slight decrease in terms of classification.



\begin{figure}[t]
	\small
	\setlength{\abovecaptionskip}{-0.1cm}
	\setlength{\belowcaptionskip}{-0.4cm}
	\centering
	\includegraphics[width=0.37\textwidth]{resources/stationary_acm_P1_JS}
	\caption{\small Variation of node distribution during meta-path ``APVPA'' guided random walks on the ACM dataset.}
	\label{Fig:stationary_analysis_P1}
%	\vspace{-0.3in}
\end{figure}







%\subsection{Case Study: Efficiency Analysis}
%\label{sec:Speedup}
%In this section, we further compare the efficiency of
%with % standard random walk used in Metapath2vec.
%traditional meta-path/meta-graph constrained no-spacey random walk (as used in Metapath2vec and Metagraph2vec).
%We first follow the settings of Section~\ref{sec:Parameter_Sensitivity} to test the parameter sensitivity of metapath2vec and metagraph2vec, and the results are shown as the green lines in Figure XXX.
%To intuitively demonstrate the efficiency and effectiveness of the proposed ``spacey'' strategy,
%we also follow the settings of Section~\ref{sec:Parameter_Sensitivity} to test the effects of varying walk-times $w$ and walk-length $l$ in normal meta-path/meta-graph based algorithms (i.e., Metapath2vec and Metagraph2vec) without using ``spacey'' strategy.
%The results are shown in Figure~\ref{Fig:Parameter_sensitivity}.


%We extract a subset of AMiner data by sampling papers published in the eight-category venues and corresponding authors at a ratio of 1:200, named AMiner-5k, which contains 1,345 papers and 3,879 authors.
%Then, we conduct author nodes classification experiments on this small AMiner-5k dataset to evaluate the stationary case of \textit{PMSW-metapath} using Eq.~(\ref{Eq:KL}) to learn the node embeddings based on the stationary distribution (as introduced in Section~\ref{sec:meta-path-guided embedding}).
%For comparison, we also evaluate the \textit{PMSW-metapath} model with different walk-length $l$ (other parameters are fixed, like walk-times=1000, windows-size=7, $\alpha$=0.01).
%% Their performances in terms of Micro-F1 score are shown in Figure~\ref{Fig:result-stationary}.
%From their Micro-F1 scores shown in Figure~\ref{Fig:result-stationary},
%we can observe that \textit{PMSW-metapath} is able to achieve a competitive performance with the walk-length increasing.
%
%Notice that directly optimizing the objective function in Eq.~(\ref{Eq:KL}) is computationally expensive~\cite{TangQWZYM15}.
%% as we need to sum over all the non-zero proximity scores s(oi; oj) for a specific object oi.
%Moreover, computing the stationary distribution in Eq.~(\ref{Eq:skip-gram}) at least requires $\Theta(N^2)$ storage, which is also infeasible for large datasets.
%Therefore, as a memory-friendly alternative approximation, the proposed spacey-random-walk based method is very effective and ponderable to be scalable and parallelizable for large-scale real-world networks.






%Case Study: Scalability
\subsection{Complexity and Scalability Analysis}
In this section, we demonstrate the scalability of the proposed frameworks by measuring both the walk time to generate heterogeneous neighborhood and the training time to learn node embeddings.
%memory usage on HINs with different sizes.
We first follow the meta-schema of DBLP network to simulate a series of random graph datasets with the average degree of 10.
The specific network sizes are [1k; 10k; 100k; 1000k; 10000k].
%Then, we use the default settings (as shown in Sec.~\ref{sec:exp_settings}) 
Then, we independently run experiments on these synthetic HINs in a computing server with $56$ core Intel(R) Xeon(R) CPU E5-2680 v4 @ 2.40GHz. % and use $50$ CPU core (one thread in one core).
The time consumption is shown in Figure~\ref{Fig:scalability_time}, which shows that our methods all have a linear time complexity with respect to the number of nodes and can be easily applied to very large-scale networks.
In fact, 
%for the walk phase, our proposed spacey random walk is quite parallelizable and efficient for large-scale networks, shown as the normal random walk used in DeepWalk~\cite{PerozziAS14}.
%no essential difference
for the random walk phase in an HIN ${\mathcal G} = ({\mathcal V}, {\mathcal E}; \mathcal A, \mathcal R)$ with  walk-times $t$ and walk-length $l$,
the spacey walk for each step takes $O(|\mathcal A|)$ time, and the total walk complexity is $O(wl|\mathcal A||\mathcal V|)$, which is linear to the number of nodes.
For the training phase, we use a Skipgram model to train the embeddings of different types of nodes, which also has a linear complexity  and can be parallelized by using the same mechanism as word2vec~\cite{GroverL16}.
%The proposed spacey random walk is also easy to be parallelized for large-scale networks.
Overall, the proposed algorithms are quite efficient and scalable for large-scale heterogeneous networks.


%In \textit{PMSW-metapath} and \textit{PMSW-metaschema}, we use a Skipgram model to train the embeddings of different types of nodes, which has no essential difference with standard Skipgram model introduced in word2vec~\cite{Mikolov2013} and can be parallelized by using the same mechanism as word2vec and Node2vec~\cite{GroverL16} and be used in very large scale network embedding.
%Furthermore, we use the spacey random walk to approximate the higher-order Markov matrix, which is also computationally efficient for both space and time complexity. 
%The random walk is also easy to be parallelized for large-scale networks.
%In this section, we extract a series of datasets of different scales from AMiner at different sampling ratios (Similar as AMiner-5k dataset in Section~\ref{Stationary-Analysis}) to compare the personalized spacey random walk used in our models with standard random walk used in Metapath2vec.
%% demonstrate the scalability of the proposed models. 
%The specific values are [1k; 5k; 10k; 50k; 100k; 500k; 1000k; 5000k].
%We run experiments in a computing server with $56$ core Intel(R) Xeon(R) CPU E5-2680 v4 @ 2.40GHz. And for each of them, we set the parameters as walk-times $w$=500, walk-length $l$=100, window-size $k$=7,
%personalized probability $\alpha$=0.01, and using $50$ CPU core (one thread in one core).
%The time consumption and memory usage during the random walk process are shown in Table~\ref{Tab:Scalability}.
%We can see that the personalized spacey random walk will not cause additional time and memory consumption.
%Overall, the proposed \textit{PMSW-metapath} and \textit{PMSW-metaschema} are quite efficient and scalable for large-scale heterogeneous networks.





\begin{figure}[t]
	\small
	\setlength{\abovecaptionskip}{-0.1cm}
	\setlength{\belowcaptionskip}{-0.4cm}
	\centering
	\includegraphics[width=0.45\textwidth]{resources/scalability_time}
	\caption{\small The walk and train time of the proposed models over different network sizes.}
	\label{Fig:scalability_time}
\end{figure}


















==> v5 - for arxiv/framework.tex <==

\section{Heterogeneous Spacey Random Walk based Embeddings}\label{sec:frameworks}
In this section, we introduce the general HIN embedding frameworks for a meta-path, a meta-graph, and a meta-schema.
%All of them are capable of learning semantically meaningful embeddings for multiple types of nodes in an HIN.
%In this section, we propose three general scalable HIN embedding algorithms: {\it SpaceyMetapath}, {\it SpaceyMetagraph}, and  {\it SpaceyMetaschema}, guided by a meta-path, a meta-graph and a meta-schema, respectively. 

%\vspace{-0.05in}
\subsection{Meta-path based HIN Embedding}
\label{sec:spaceymetapath}
%Given a meta-path, we first define the general meta-path count based  proximity (similarity) for any pair of entities in the HIN.
% For simplicity, we use type names connected by ``$-$'' to denote the meta-path when there are no multiple relations between a pair of types: $\mathcal P = {\it (A_1-A_2- \ldots -A_{L+1})}$.
%
% To see how a meta-path can affect the similarities between entities, we define the following CountSim similarity given a meta-path.
%
%\begin{definition}
%\label{def:countsim}
%{\it \textbf{CountSim}. 
%Given a meta-path $\mathcal P = (A_1-A_2- \ldots -A_{L+1})$, CountSim is a function of the count of path instances:
%%\begin{equation}
%%		{\small
%		$	{\rm CountSim}_{\mathcal P}(v_i,v_j) \triangleq {\bf M}_{\mathcal P}(v_i,v_j) = {\bf W}_{A_1A_2} \cdot {\bf W}_{A_2A_3}\cdot \ldots \cdot{\bf W}_{A_{L}A_{L+1}},
%			\label{eqn:ps}
%		$
%%		}
%%%\end{equation}
%where ${\bf W}_{A_kA_{k+1}}$ is the adjacency matrix between types $ A_k$ and $ A_{k+1}$ in meta-path $\mathcal P$.
%}
%\end{definition}
% \vspace{-0.05in}
%The number of path instances between $v_i$ and $v_j$ following $\mathcal P$ is ${\rm CountSim}(v_i,v_j) = |\{p_{{i}\rightsquigarrow{j}} \in \mathcal P\}|  = {\bf M}_{\mathcal P}(v_i,v_j)$.
%For example, for author similarity based on papers, the composite relation {\it two authors co-authoring same papers} can be described as {\it Author-Paper-Author} (APA) for simplicity.
%This meta-path simply gives us ${\bf M}_{{\mathcal P}_{APA}}={\bf W}_{AP} {\bf W}_{AP}^T$, which is the dot product between author vectors represented by a bag of papers, where ${\bf W}_{AP}$ is the author-paper co-occurrence matrix.


% Our goal is to find a semantically meaningful entity representations for all entities under the constraint of meta-path $\mathcal P$.
% A straightforward method is to directly perform matrix factorization over the matrix computed by ${\rm CountSim}(v_i,v_j)$, which has been used by~\cite{HuanZhao2017}.
% However, such a way absorbs all the other entity type information into $A_1$ and $A_{L+1}$ in meta-path $\mathcal P$.
% Recently, network embedding based random walk has been developed~\cite{PerozziAS14,GroverL16}, and it can be applied to very large scale networks.
% Random walk based algorithms correspond to factorization of a matrix defined by exploring higher-order proximities in a network's topology~\cite{YangSLT17}.
% It is also known that in the extreme case with an infinity context, random walk based embedding approaches can be formulated as using node embeddings to approximate the convergent distribution of personalized PageRank~\cite{ChoBP15}.
%If the count is not normalized for different meta-paths, it is difficult to compare over different meta-path based similarities.
%Thus, people have thought about the ways of normalization.
%One way of normalization is called PathSim~\cite{Yizhou11}, where the count based similarity ${\bf M}_{\mathcal P}(i,j)$ is normalized by the count based similarities of each entity ${\bf M}_{\mathcal P}(i,i)$ and ${\bf M}_{\mathcal P}(j,j)$.


Given an arbitrary meta-path $\mathcal P \!= \!{\it (A_1\!\to \!A_2\!\to\! \ldots \!\to \!A_{L\!+\!1})}$,  our goal is to learn the semantically meaningful embeddings for all entities under the constraint of $\mathcal P$.
%As first, to see how a meta-path $\mathcal P$ affect the similarities between entities, we can compute the commuting matrix ${\bf M}_{\mathcal P}$ (as defined in Def.~\ref{def:commuting_metapath}), which measures the general meta-path count based  proximity (similarity) for any pair of entities in the HIN.
%Then, a straightforward method is to directly perform matrix factorization over the matrix ${\bf M}_{\mathcal P}$
%, which has been used by
%\cite{HuanZhao2017}.
%However, such a way absorbs all the other entity type information into $A_1$ and $A_{L+1}$ in meta-path $\mathcal P$, and are costly for computation and memory.
%Recently, network embedding based random walk has been developed~\cite{PerozziAS14,GroverL16}, and it can be applied to very large scale networks,
%Random walk based algorithms correspond to factorization of a matrix defined by exploring higher-order proximities in a network's topology~\cite{YangSLT17}.
%which is also known that in the extreme case with an infinity random-walked context, the random walk based embedding approaches can be formulated as using node embeddings to approximate the convergent distribution of personalized PageRank~\cite{ChoBP15}.
We proceed by extending the meta-path guided random walk based embedding~\cite{YuxiaoDong2017} in view of the scalability for large-scale networks.


\subsubsection{Background of Random Walk over HIN}
Meta-path guided random walk over an HIN was first considered in computing similarities in the path ranking algorithm (PRA)~\cite{LaoC10}.
%The other way to normalize the commuting matrix is used in the path ranking algorithm (PRA)~\cite{LaoC10}.
%In PRA, it normalizes the individual adjacency matrix ${\bf W}_{\cdot}$.
%It assumes the normalized adjacency matrix defines transition probabilities:
It defines the following transition probabilities:
%\vspace{-0.05in}
\begin{equation}\label{Eq:normalized_adjacency_matrix}
{\bf P}_{\!A_l,A_{l+1}} = {\bf D}_{\!A_l,A_{l+1}}^{-1}{\bf W}_{\!A_l,A_{l+1}},
\end{equation}
%\vspace{-0.1in}
%where ${\bf W\!}_{\!A_l\!,A_{l+1}}\!\!\! \in \!\!{\mathbb R}^{\!|\!{\mathcal V}_{\!A_l}\!|\times |\!{\mathcal V}_{\!A_{\!l+1}}\!|\!}$   is  the adjacency matrix between nodes in types $A_l$ and $A_{l+1}$, % nodes in type $ A_{l+1}$,
where ${\bf W\!}_{\!A_l\!,A_{l+1}}$ is the adjacency matrix between nodes in type $A_l$ and nodes in type $ A_{l+1}$,
and ${\bf D\!}_{\!A_l,A_{l+1}}$ is the degree matrix with  ${\bf D\!}_{\!A_l,A_{l+1}}\!(v_i,\!v_i) \!\!=\! \!\!\sum_j \!\!{\bf W\!}_{\!A_l\!,A_{l+1}}\!(v_i,\!v_j)$.
When performing a random walk from a node $v_i$ in type $A_l$, we choose next node $v_j$ in type $A_{l+1}$ based on the probability ${\bf P}_{\!A_l,A_{l+1}}(\!v_i,\!v_j)$.
In PRA algorithm, it uses the normalized commuting matrix, i.e., ${\bf P\!}_{\!A_1\!,A_2} \!\!\cdot\! {\bf P\!}_{\!A_2\!,A_3}\!\!\cdot\! \ldots \!\cdot \!{\bf P\!}_{\!A_{\!L}A_{\!L+1}}$ to define the meta-path based similarities between nodes of type $A_1$ and $A_{L+1}$,
and claims that this is an ad-hoc definition of hitting/commuting probability. %for nodes with types $A_1$ and $A_{L+1}$.
The actual expected hitting/commuting probability can be approximated by the stationary distribution of the random walk following the meta-path constraints.
%By deploying random walk, such probability is exactly simulated by the expected hitting/commuting times of the meta-path constrained Markovian random walks in the limiting stationary case.
%However other nodes with types $A_{l} (l\neq 1, L+1)$ have not been considered and the similarities are not exactly the expected hitting/commuting probabilities.
However, as discussed in Section~\ref{sec:introduction},
the existing random walk based HIN embedding methods (e.g.,~\cite{YuxiaoDong2017,FuLL17,ChuanShi2017,zhang2018metagraph2vec}) directly use the random walk sampling but pay few attention to definitely explore the higher-order Markov chain property of meta-path guided random walk, especially to its limiting stationary distribution, which is essential for describing the long-run behavior of the random walk.
%As a result, their random walk simulations, though generating the correct walk path constrained by the meta-path, may be insensitive and ineffecient to be stationary.


\subsubsection{Higher-order Markov Chains}
In this section, 
we first clarify that the meta-path guided random walk is a higher-order Markov chain using the following lemma and its explanations.
% Then, we present a non-Markovian spacey random walk to %more efficiently and effectively approximate the meta-path guided higher-order Markovian random walk.
% improve the walk effectiveness and efficiency, which is mathematically guaranteed to attain the same limiting stationary distribution of the normal meta-path guided higher-order Markovian random walk~\cite{BensonGL17}.
% % After that, we also follow the principles of random walk based network embedding~\cite{PerozziAS14} to develop a meta-path based HIN embedding model by applying the spacey random walk strategy.
% %the following higher-order Markov chain based random walk.
% %% We also follow the principles of random walk based network embedding, which was first proposed in DeepWalk~\cite{PerozziAS14}, which consists of two steps: first, it performs random walk on the HIN nodes guided by a meta-path; second, it runs Skipgram algorithm~\cite{Mikolov2013} to use a center node in the random walk path to predict its context nodes.
% %Since we can compute the stationary distribution  of our higher-order Markov chain, we can provide an extreme case of the network embedding, where the network embedding is used to approximate the expected commute time between nodes based on a personalized random walk.
% %In the following, we will introduce the expected commute time for the personalized random walk, and then derive a DeepWalk-type algorithm to handle large-scale networks.
% %\subsubsection{Arbitrary Meta-path based Higher-order Markov chain}
% %Before that, 
% The following lemma is used to formalize the meta-path based higher-order Markov chain.

%\vspace{-0.05in}
\begin{lemma}\label{lemma:meta_path_Markov_property}
{\it
%Any meta-path can be used to define a higher-order Markov chain. Then the Markov chain can be used to guide a random walk %with a stationary distribution.
%constrained by the meta-path.
For an arbitrary meta-path $\mathcal P \!=\! {\it (A_1\!\to\! A_2\!\to\! \cdots \!\to\! A_{\!L+\!1})}$, 
we can define a $k$th-order Markov chain, iff $\mathcal P$ can be divided into a set of unique $k$-length meta-paths ${\it (\!A_l\!\to\! A_{l+1}\!\to\! \cdots \!\to \!A_{l+\!k})}$ which satisfy that if the last $k$ states are determined by ${\it (A_l, A_{l+\!1}, \cdots\!, A_{l+\!k-\!1})}$, the current state can only be $A_{l+k}$.
After that, we can obtain the transition probabilities of the $k$th-order Markov chain by concatenating the normalized commuting/adjacency matrix of these $k$-length meta-paths, and such transition probabilities can be used to guide a random walk constrained by $\mathcal P$. 
}
\end{lemma}
%\vspace{-0.05in}
Note that to ensure the random walk runs continuously, we generally regard $\mathcal P$ should be cyclic with the same start and end entity types, i.e., $A_1 \!=\! A_{L+1}$ (If not, it is easy to jump back from either start or end to get a symmetric one).
Taking the meta-path %``{\it Author$\to$Paper$\to$Venue$\to$Paper$\to$Author} (APVPA)'' 
``APVPA'' illustrated in Figure~\ref{Fig:A_HIN} as an example,
we can divide ``APVPA'' into a set of meta-paths: ``APV'', ``PVP'', ``VPA'', and ``PAP''.
With these factorized meta-paths, walking to the current state is uniquely determined by the last two states.
For example, if and only if the last state is a {\it paper} (P) and the second last state is an {\it author} (A), the current state can be only determined to be a {\it venue} (V).
Thus %the ``APVPA'' guided random walk can essentially be defined as a second-order Markov chain process.
a second-order Markov chain can be used to represent the ``APVPA'' guided random walk.
% when we need to perform random walk from ``P'' to another type of node, there are two choices, ``V'' and ``A''. Given the previous type before ``P'' being ``A'' or ``V,'' the random walk should be different.
Further, we can define a hypermatrix (three-dimensional tensor) to denote the transition probability for such second-order Markovian random walk.

\begin{definition}
{\it
A second-order hypermatrix ${\bf H}$ for the meta-path guided second-order Markovian random walk can be defined as:
%\vspace{-0.05in}
\begin{equation}\label{Eq:second_order_transition_hypermatrix}
{\bf H}_{i,j,k} \triangleq \left\{ 
\begin{aligned}
& \phi(v_i)=A_l, \\
{\bf P}_{A_{l+1},A_{l+2}}(v_j,v_k),\ \ \  & \phi(v_j)=A_{l+1}\\
& \phi(v_k)=A_{l+2} \\
0,  otherwise &
\end{aligned}
\right.,
\end{equation}
%\vspace{-0.05in}
where ${\bf H}_{i,j,k}$ represents the transition probability to node $v_k$, given the last node $v_j$ and the second last node $v_i$;
``$A_lA_{l+1}A_{l+2}$'' is one of  ``APV'', ``PVP'', ``VPA'', or ``PAP''; $\phi(\cdot)$ is the node type mapping; and ${\bf P}_{A_{l+1},A_{l+2}} $ is defined as Eq. (\ref{Eq:normalized_adjacency_matrix}).
}
\end{definition}


%After the above formalization of the meta-path guided higher-order Markovian random walk,
Although we have formalized the meta-path guided higher-order Markovian random walk,
there can be some trivial walks.
Due to the nature of higher-order Markov chain, the transitions following a meta-path usually depend on the last several states rather than just the last one. As a result, an entity may play a redundant role in the walks.
%For example, as illustrated in Figure~\ref{Fig:A_HIN}, for the random walks guided by the ``APVPA'' meta-path, we will constrain that  for the first ``P'' in the meta-path, the next node must be ``V'' and for the second ``P'' in meta-path, the next node must be ``A''. That is, when we perform next walk from a ``P'', we need to know the previous state before ``P'' is ``A'' or ``V'' to judge the ``P'' is the first or the second. Thus, this is theoretically a second-order Markov chain because the transitions depend on the second last state, rather than just the last one.
%when we need to perform random walk from ``P'' to another type of node, there are two choices, ``V'' and ``A''. Given the previous type before ``P'' being ``A'' or ``V,'' the random walk should be different.
%For example, if the last state is a {\it paper} (P), and the second last state is an {\it author} (A), then the current state can only be determined to be a {\it venue} (V).
For example, we define the meta-path ``APVPA'' based second-order Markovian random walk to extract the author similarity by the semantic ``Two authors published at a venue'', and the walk path instances are illustrated in Figure~\ref{Fig:A_HIN}(a).
Among them, %these path instances, 
we can find the red one $a_1\!\!\to\! \!p_1\!\!\to\!\! v_1\!\!\to\!\! p_1\!\!\to \!\!a_2$ actually expresses the same information as the path instance $a_1\!\!\to \!\!p_1\!\!\to\!\! a_2$ following  ``APA''.
In this case, the intermediate transitions $p_1\!\!\to \!\!v_1\!\!\to\!\! p_1$ are trivial walks and can be skipped, 
i.e., %which means that 
when we walked from an author $a_1$ to a paper $p_1$, we then can immediately skip to another author as if the current $p_1$ was just walked from a venue $v_1$.
Such shortened walk path $a_1\!\!\to \!\!p_1\!\!\to\!\! a_2$ can be regarded as a faster instance of meta-path ``APVPA''.
This fact motivates us that instead of strictly constraining the walks by the meta-path, it can be preferred to occasionally skip the intermediate trivial transitions with a principled probability.
Then, the meta-path based higher-order Markovian random walk can be more efficient to attain the expected stationary distribution.
Intuitively, for any meta-path $\mathcal P^* \!\!=\!{\it (A_1\!\to\!\cdots\! A_l\!\to\! \cdots \!A_k\!\cdots \!\to\!\! A_{\!L+\!1})}$ with $A_l\!=\!A_k$, we can probabilistically perform a faster random walk following the folded meta-path ${\it (A_1\!\to\!\cdots\! A_l\!\to \!A_{k+\!1}\!\cdots \!\to\! A_{\!L+\!1})}$, and the walk path can be equivalently regarded as a special instance of meta-path $\mathcal P^*$.
%Therefore,
%for better efficiency and effectiveness, 
%we next introduce a spacey random walk~\cite{BensonGL17} to improve the normal meta-path based higher-order Markovian random walk.
To achieve this, we introduce the following spacey random walk strategy.


\subsubsection{Heterogeneous Personalized Spacey Random Walk}
Given a % homogeneous 
higher-order Markov chain, % and associated transition hypermatrix,
the spacey random walk provides a space-friendly and efficient alternative approximation and is mathematically guaranteed to converge to the same limiting stationary distribution~\cite{li2014limiting,BensonGL17}.
Inspired by that, 
to obtain the embeddings of multi-typed entities in an HIN, we first define our meta-path based heterogeneous personalized spacey random walk (called {\it HeteSpaceyWalk}) as follows.
We use the aforementioned ``APVPA'' based second-order Markov chain and transition hypermatrix ${\bf H}_{i,j,k}$ as an illustration, while higher-order chains are similar.

\begin{definition}\label{def:personalized_spacey_walk}
{\it \textbf{Heterogeneous Personalized Spacey Random Walk for a Meta-path based Second-order Markov Chain}.
Given a second-order Markov chain, the transition hypermatrix ${\bf H}_{i,j,k}$ is concatenated by a set of transition probabilities based on a set of factorized meta-paths (as defined in Eq. (\ref{Eq:second_order_transition_hypermatrix})).
Then, these  transition probabilities can be used to guide a personalized spacey random walk.
%We denote the  random walk rooted at a node $v_0$ as a stochastic process with a sequence of random variables $W_{v_0}(0), W_{v_0}(1), W_{v_0}(2),\cdots \!,W_{v_0}(n)$, and the probability law to guide our heterogeneous spacey random walk is defined to use:
%The probability law of the personalized spacey random walk is to use:
%Such stochastic process consists of a sequence of states/nodes $X(0), X(1), X(2),\cdots \!,X(n)$, and the probability law is defined to use an occupation probability:
Such stochastic process consists of a sequence of states/nodes $X(0), X(1), X(2),\cdots \!,X(n)$, and the probability law is defined to use
%\vspace{-0.05in}
\begin{equation}\label{Eq:spacey_out_law}
Pr\!\left\{Y(n)\!=\!v_i | \mathcal{F}_n \right\} \triangleq
\begin{cases}
(1-\alpha) + \alpha{\bf w}_i(n), &v_i=X(n-1) \\
\alpha{\bf w}_i(n), & v_i\not =X(n-1) 
\end{cases}
\end{equation}
to choose the second last state $Y(n)$, and then use
%\vspace{-0.05in}
\begin{equation}\label{Eq:spacey_walk}
Pr\!\left\{X(n+1)=v_k | X(n)=v_j, Y(n)=v_i \right\}  \triangleq  {\bf H}_{i,j,k}
\end{equation}
to choose the next node, where $\mathcal{F}_n$ is the $\sigma$-field generated by the random variables $X(i), i\!=\!1,2,...,n$, $X(0)$ is the initial state; 
$\alpha \in (0,1)$  is a hyper-parameter that can control a user's personalized behavior;
%$\alpha \in (0,1)$ is a parameter controlling the probability of returning to the starting state with probability $\alpha$ and moving to next state following second-order Markov chain with probability $1-\alpha$.
${\bf w}(n)$ is the occupation vector at step $n$ and is defined as:
%\vspace{-0.05in}
\begin{equation}\label{Eq:occupation_vector}
{\bf w}_i(n) \triangleq \frac{1}{n+ N}\left( 1+\sum_{s=1}^{n} Ind\left\{X(s)=v_i\right\}\right),
\end{equation}
where $N$ is the number of total states.
}
\end{definition}
% In the personalized spacey random walker process on HIN
In short, 
with personalization, once the spacey random walker visits $X(n)$ at step $n$, it spaces out and forgets its second last state (i.e., the state $X(n-1)$) with probability $\alpha$.
It then invents a new history state $Y(n)$ by randomly drawing a past state $X(1),...,X(n)$.
Then it transitions to $X(n+1)$ as if its last two states were $X(n)$ and $Y(n)$.
Without personalization (i.e. $\alpha\!=\!0$), the spacey random walker performs a normal second-order Markovian random walk.



%\begin{figure*}
%	\vspace{-0.1in}
%	\setlength{\abovecaptionskip}{-0.1cm}
%	\setlength{\belowcaptionskip}{-0.4cm}
%	\centering
%	\subfigure[\small Meta-path based Markovian random walk.]{
%		\label{Fig:Markovian_random_walk}
%		\includegraphics[width=0.4\textwidth]{resources/Markovian_random_walk}
%		%		\vspace{-0.1in}
%	}
%	%     \hfill
%	\hspace{0.2in}
%	%	    \vspace{0.0in}
%	\subfigure[\small Meta-path based spacey random walk.]{
%		\label{Fig:spacey_random_walk}
%		\includegraphics[width=0.5\textwidth]{resources/spacey_random_walk}
%	}
%	%\vspace{-0.1in}
%	\caption{\small An intuitive comparison of meta-path based Markovian random walk and spacey random walk, given the meta-path ``APVPA'' on the scholar network illustrated in Figure~\ref{Fig:A_HIN}(a).
%In short, when the spacey random walker transitioned from ``P'' to the next,  it forgets its second last state is ``A'', and then uses Eq.~(\ref{Eq:spacey_out_law}) to choose a new history state which is assumed as the precursor of ``P''.
%Constrained by ``APVPA'' based second-order Markov chain, the assumed precursor of ``P'' can be ``V'' or ``A'', and respectively, there are two rules to guide the next transition: direct transition to ``A'' ({\it rule1}), or transition to ``V'' as a normal ``APVPA'' based second-order Markovian random walk ({\it rule2}).
%}
%	\label{Fig:comparison_random_walk}
%\end{figure*}
\begin{figure*}
	\small
	\vspace{-0.1in}
	\setlength{\abovecaptionskip}{-0.1cm}
	\setlength{\belowcaptionskip}{-0.4cm}
	\centering
	\includegraphics[width=0.9\textwidth]{resources/comparison_markov_spacey}
	\caption{\small An intuitive comparison of meta-path based Markovian random walk and spacey random walk.
%		given the meta-path ``APVPA'' on the scholar network illustrated in Figure~\ref{Fig:A_HIN}(a).
%		In short, 
		When the spacey random walker walks from ``P'' to the next,  it forgets its second last state is ``A'' and uses Eq.~(\ref{Eq:spacey_out_law}) to choose a new state which is assumed as the precursor of ``P''.
		Constrained by ``APVPA'' based second-order Markov chain, the assumed precursor of ``P'' can be ``V'' or ``A'', and respectively, there are two rules to guide the next transition: directly walk to ``A'' ({\it rule1}), or walk to ``V'' as a normal Markovian random walk ({\it rule2}).
	}
	\label{Fig:comparison_random_walk}
%	\vspace{-0.2cm}
\end{figure*}



Figure~\ref{Fig:comparison_random_walk} shows an intuitive example of comparing normal meta-path based Markovian random walk and our proposed meta-path based spacey random walk, given the meta-path ``APVPA'' on the scholar network illustrated in Figure~\ref{Fig:A_HIN}(a).
We can see that, different from the Markovian random walk which strictly follows the constraints of the user-given meta-path,
the spacey random walk allows skipping the intermediate transitions to improve walk efficiency and quality, which is actually a shortened random walk following the folded sub-path of the original user-given meta-path.
In fact, as illustrated in Figure~\ref{Fig:comparison_random_walk}(b),
the spacey strategy produces a special meta-graph/multi-meta-paths (which we call as the {\it meta-path based spacey graph} integrating the original user given meta-path and its folded sub-meta-paths) guided random walk process.
%And we denote such special meta-graph/multi-meta-paths as the {\it meta-path based spacey graph}.
As a result, the proposed spacey random walk can efficiently and effectively capture richer information and thus achieve better performance than the normal Markovian random walk.
For example, we can see the two walk instances in Figure~\ref{Fig:comparison_random_walk}, which indicate that the spacey random walk can use shorter walk steps to capture richer relationships than normal Markovian random walk.
Moreover,
different from directly deploying meta-graph/multi-meta-paths guided random walk, which is problematic to determine appropriate proportions to balance multiple meta-paths,
the proposed spacey random walk adaptively adjusts the probability of following  the original meta-path or any folded sub-meta-path  according to  a carefully designed personalized occupation probability (as defined in Eq.~(\ref{Eq:spacey_out_law})) calculated dynamically by past states.
The following theorem shows the guarantee of
only more efficiently and effectively extracting the specific semantic of domain-proficient meta-path provided by users, i.e., the proposed spacey strategy will not absorb other heterogeneous information beyond the users' concern.
\begin{theorem}\label{theorem-convergence}
The limiting distribution of the heterogeneous personalized spacey random walk for a meta-path equals to the same stationary distribution of the original meta-path based higher-order Markovian random walk under the rank-one approximation condition.
\end{theorem}

%Due to the lack of space, the proof of the theorem is shown in Appendix~\ref{appendix-proof} in the supplementary material. $\blacksquare$

The proof follows the spacey random walk theory~\cite{BensonGL17} and  $z$ eigenvector solution theory~\cite{li2014limiting} which point out that by considering a ``rank-one approximation'' for a transition hypermatrix ${\bf H}$ of second-order Markov chain, the stationary distribution formula reduces to
%According to the $z$ eigenvector solution theory~\cite{li2014limiting} which points out that the stationary distribution formula for a transition hypermatrix can be reduced to:
\begin{equation}
{\bf \pi}_k = \sum_{i,j}{\bf H}_{i,j,k}{\bf \pi}_j {\bf \pi}_i, \ \ \sum_k {\bf \pi}_k =1, {\bf \pi}_k \ge0, N\ge k\ge 1,
\end{equation}
where ${\bf \pi}_k$ is node distribution and $N$ is the number of nodes.
Following this,
we next demonstrate that the unique stationary solution of meta-path based second-order Markov chain is also the limiting distribution of the proposed personalized spacey random walk.

First, we can formally express that the defined spacey random walker $\{X(n)\}$ approximates a second-order Markov chain with a first-order transition probability matrix:
\begin{equation}\label{Eq:probabilities_matrix_spacey_walk}
\begin{split}
{\bf R}_{j,k} & \triangleq \sum_i {\bf H}_{i,j,k}\left( (1-\alpha){\bf x}_i(n)+\alpha{\bf w}_i(n) \right) \\
& = [{\bf H}\cdot(((1-\alpha){\bf x}(n) + \alpha{\bf w}(n))\otimes {\bf I})]_{j,k},
\end{split}
\end{equation}
where ${\bf x}(n)$ is the nodes distribution at step $n$, ${\bf w}(n)$ is the occupation probability vector at step $n$ (as defined in Eq.~(\ref{Eq:occupation_vector})).

Then,
%suppose that
if the process  $\{X(n)\}$  converges to a unique stationary distribution ${\bf x}(n)$ satisfying ${\bf R}{\bf x}(n)={\bf x}(n)$,
for the case  $n\gg L > 0$, we have:
\begin{equation*}
{\bf w}(n+L) \thickapprox \frac{n{\bf w}(n)+L{\bf x}(n)}{n+L}={\bf w}(n)+\frac{L}{n+L}({\bf x}(n)-{\bf w}(n)).
\end{equation*}
In a continuous time limit $L\to 0$, we have:
\begin{equation*}
\frac{d{\bf w}(n)}{dL}\thickapprox \lim_{L\to 0} \frac{{\bf w}(n+L)-{\bf w}(n)}{L}=\frac{1}{n}({\bf x}(n)-{\bf w}(n)).
\end{equation*}
Thus,  if this process converges, it must converge to a point where ${\bf x}(n)={\bf w}(n)$.
Further, we can find that the limiting distribution ${\bf x}$ heuristically satisfy:
\begin{equation*}
{\bf x}={\bf R}{\bf x}={\bf H}\cdot({((1-\alpha){\bf x}+ \alpha{\bf w})}\otimes {\bf I}){\bf x}={\bf H}\cdot({\bf x}\otimes {\bf I}){\bf x}={\bf H}\cdot({\bf x}\otimes {\bf x}).
\end{equation*}
%\vspace{-0.05in}
That is,
%\vspace{-0.01in}
\begin{equation*}
{\bf x}_k=\sum_{i,j}{\bf H}_{i,j,k}{\bf x}_j {\bf x}_i.
\end{equation*}

Therefore, the limiting distribution of matrix $ {\bf R}$  is also the unique stationary solution of hypermatrix ${\bf H}$.
The defined heterogeneous personalized spacey random walk provides an efficient alternative approximation for the meta-path based higher-order Markovian random walk without changing the limiting stationarity.






\subsubsection{Spacey Random Walk based Embedding}
Now we can use the heterogeneous personalized spacey random walk to generate node sequences in an HIN, and then feed them to the Skipgram model~\cite{mikolov2013efficient,Mikolov2013} to learn node embeddings.
% %Given a node $v$ in an HIN  ${\mathcal G} = ({\mathcal V}, {\mathcal E};{\mathcal A}, {\mathcal R})$,
% %we seek to optimize the following objective function, which maximizes the log-probability of having the heterogeneous neighborhoods $N_A(v)$, $A \in {\mathcal A}$.
% % Given the results in~\cite{YangSLT17}, it is easy to show that the existing random walk based algorithms for HINs~\cite{YuxiaoDong2017,HuangM17,ShangQLKHP16} can all be seen as special cases of our framework where the context window used to define node context corresponds to the number of random walk iterations.
% % In addition, they can only apply to meta-paths starting and ending with the same type of entity, as is shown in Figure~\ref{fig:comparison-5}.
% % In scalable, it is known that in the extreme case with an infinity context, random walk based embedding approaches can be formulated as using node embeddings to approximate the convergent distribution of personalized PageRank~\cite{ChoBP15}.
% % Therefore, 
% Specifically, given a heterogeneous network and an arbitrary meta-path as input, we run the personalized spacey random walk over all entities to generate paths of multiple types of nodes.
% % As the spacey random walk is based on a higher-order Markov chain guided by arbitrary meta-path provided by human, 
% % the heterogeneous semantic relationships between different types of entities provided by the meta-path can be naturally properly incorporated into the generated paths.
% The paths can be then as the input of Skipgram algorithm to learn the the latent representations of nodes inspired by word2vec~\cite{mikolov2013efficient,Mikolov2013}.
% % which are naturally able to capture the heterogeneous semantics of different types of entities and their relationships provided by the meta-path.
We follow~\cite{YuxiaoDong2017} to define the heterogeneous Skipgram model.
Given the generated paths corpus $\mathcal{V_P}$ guided by meta-path $\mathcal P$, the model is to minimize following objective function:
\begin{equation}\label{Eq:skip-gram}
  \mathop{\arg\min}_{\theta} \ -\sum_{v_i\in \mathcal{V_P}}\sum_{A\in \mathcal{A}}\sum_{v_j \in {\mathcal N}_A(v_i)}\log Pr(v_j|v_i,\theta),
\end{equation}
where ${\mathcal N}_A(v_i)$ denotes $v$'s neighborhood with type $A$. For each pair of entities $(v_i,v_j)$, their joint probability $Pr(v_j|v_i,\theta)$ is commonly defined as such softmax function:
\begin{equation}\label{Eq:softmax}
Pr(v_j|v_i,\theta) = \frac{\exp\{{\bf u}_j^T {\bf v}_i\}}{\sum_{j'}\exp\{{\bf u}_{j'}^T {\bf v}_i\}},
\end{equation}
where ${\bf u}_j$ is the context vector of $v_j$ and ${\bf v}_i$ is the embedding vector of $v_i$.
We also use the negative sampling technique~\cite{Mikolov2013} for optimizing Eq.~(\ref{Eq:skip-gram}) which is modified as: \begin{equation}\log \sigma({\bf u}_j^T {\bf v}_i\}) +
  \sum_1^m \mathbb{E}_{v_c \thicksim P_n(v_i)} \left[\log \sigma(-{\bf u}_c^T {\bf v}_i\}) \right],
\end{equation}
% \begin{equation}
% \mathop{\arg\min}_{\theta} \ -\sum_{v_i\in \mathcal{V_P}}\sum_{A\in \mathcal{A}}\sum_{v_j \in N_A(v_i)}
%   \left(
%   \log \sigma({\bf u}_j^T {\bf v}_i\}) +
%   \sum_1^k \mathbb{E}_{v_c \thicksim P_n(v_i)} \left[\log \sigma(-{\bf u}_c^T {\bf v}_i\}) \right] 
%   \right),
% \end{equation}
where $\sigma(x)\!=\!\frac{1}{1+\exp\{-x\}}$ and $P_n(v_i)$ is the %noise distribution to perform sampling.
sampling distribution.

%Alternatively, we can equivalently represent the cost function in Eq.~(\ref{eq:costKL}) as:
%\begin{equation}\label{Eq:KL}
%C({\bf s}, {\hat {\bf s}}) \!=\! \sum_{v_i,v_j \in \mathcal{V}} \! -{\bf s}_i^{(j)} \log \hat{{\bf s}}_i^{(j)} \!=\! -\!\sum_{v_i,v_j \in \mathcal{V}} {\bf s}_i^{(j)} \log Pr(v_j|v_i,\theta).
%\end{equation}
%Notice that the meta-path based proximity ${\bf s}_i^{(j)}$  between $v_i$ and $v_j$ could be regarded as a weight to control the training process of minimizing their joint probability.
%In this case,
%Eq.~(\ref{Eq:skip-gram}) can be regarded as an approximation to Eq.~(\ref{Eq:KL}) by sampling on an HIN based on personalized spacey random walk to approximate ${\bf s}_i^{(j)}$.
%In the extreme case of personalized spacey random walk, where the walk convergences to its stationary distribution, 
%the {\it PMSW-metapath} method is equivalent to the way to minimizing the KL-divergence of the probability distributions, 
%which is also consistent with the homogeneous case and first-order Markov chain case~\cite{ChoBP15}.


We call the above approach as {\it SpaceyMetapath} algorithm.
% By leveraging the personalized spacey random walk to generate the heterogeneous neighborhood, and incorporating them to the Skipgram model, 
% {\it SpaceyMetapath} is able to efficiently and effectively produce semantically meaningful node embeddings in an HIN given the constraint of an arbitrary meta-path. 
%which preserving both the semantic and structural correlations between different types of nodes.




\subsection{Meta-graph based HIN Embedding}
% \vspace{-0.05in}
\label{sec:spaceymetagraph}

In this section, 
%given the  general meta-path based spacey random walk framework  developed in Section~\ref{sec:spaceymetapath}, 
we further propose a meta-graph based spacey random walk algorithm, named  {\it SpaceyMetagraph}.
%we extend the general meta-path based spacey random walk framework  developed in section~\ref{sec:spaceymetapath} to an arbitrary meta-graph.
Compared with single meta-path, a meta-graph can capture more complex heterogeneous structures and richer semantics by integrating multiple meta-paths.
%Thus,  the {\it SpaceyMetagraph} algorithm is able to produce more effective HIN-embeddings.
%Given an arbitrary meta-graph, it can be seen as an integration of multiple meta-paths, and these meta-paths can be used to define higher-order Markov chains. 
The challenge is how to concatenate these different higher-order Markov chains with appropriate proportions, i.e., how to balance the branch %multi-oriented 
choices in a meta-graph.
For example, for the meta-graph in Figure~\ref{Fig:A_HIN}(d), %which integrates two meta-paths: ``APVPA" and ``APTPA", we can follow Lemma~\ref{lemma:meta_path_Markov_property} to define two second-order Markov chains by factorizing the two meta-paths into a set of sub-meta-paths:  APV, PVP, VPA, APT, PTP, TPA, and PAP.
%However, when we need to perform random walk from the first ``P" to its successors, there are still two choices: ``V" or ``T''.
when we need to perform random walk from the first ``P" to its successors, there are two choices: ``A" or ``V''.
Unlike a higher-order Markovian transition, this transition does not depend on any previous state.
%Thus, we must develop a new random walk strategy to balance these multi-oriented choices, which distinguishes the meta-graph based algorithm from previous meta-path based algorithm.
%
%We first define a meta-graph based integrated higher-order Markov chain as follows:
%\begin{lemma}\label{lemma:meta_graph_Markov_property}
%	{\it
%		Any meta-graph can be used to define an integrated higher-order Markov chain with an integrated transition hypermatrix.
%	}
%\end{lemma}
%Given an arbitrary meta-graph, we can reversely divide it into multiple meta-paths which do not contain each other, and then
%we can follow Lemma~\ref{lemma:meta_path_Markov_property} to define multiple $k$th-order Markov chains  by factorizing these meta-paths into a set of $k$-length meta-paths.
%However, there is no principled way to balance these multi-oriented choices.
To deal with this issue, we extend our spacey random walk principle from choosing previous states to choosing the branch choices,
%For example, when we perform random walk from ``P'' to ``A" or ``V'', we can choose one according to their occupation distribution instead of a uniform selection.
%As a result, the meta-graph based heterogeneous personalized spacey random walk can be defined as follows.
and define our meta-graph based heterogeneous personalized spacey random walk as follows.

%We use the meta-graph in Figure~\ref{Fig:A_HIN}(d) as an illustration which consists of two meta-paths and can define two second-order Markov chains, while other meta-graphs are similar.



%That is, the meta-graph guided random walk has the same higher-order Markov property as the meta-path guided  random walk.
%For example, we can see the meta-graph in Figure XXX, which consists of two meta-paths: ``APVPA" and ``APTPA". 
%When we need to perform random walk from ``P'' to another type of node, there are two choices: ``V/T'' and ``A''. The behavior law depends on the previous type before ``P''. Thus, this is a seconder-order Markov chain.
%Then, for such meta-graph based second-order Markovian stochastic process, we can follow Def.~\ref{def:personalized_spacey_walk} to define a similar heterogeneous spacey random walk.% to efficiently and effectively  generate heterogeneous neighbors in an HIN.
%For better illustration, in Figure XXX , we distinguish the two ``P"  in the meta-graph as ``P1"  and ``P2". 
%Then,
%when we performed random walk from ``A" to ``P1'', the current walked ``P1'' can always be a ``P2'', and then we can skip the intermediate  steps between two ``P" and directly walking to ``A2".
%
%However, as a meta-graph usually has multiple meta-paths, there is a multi-orientation property which distinguishs the meta-graph guided random walk from meta-path guided random walk.
%%there is no  principled way to guide how to balance them.
%As illustrated in Figure XXX, when we exactly need to perform random walk from ``P1'' to its successors, there are  two choices: ``V" or ``T''.
%And unlike the aforementioned choice of higher-order Markov property, this choice is completely  unrelated  to the previous types.
%To deal with this issue, we extend our spacey random walk principle from choosing previous states to choosing such successors.
%For example, when  we perform random walk from ``P1'' to ``V" or ``T'', we choose one according to their occupation distribution instead of a random selection.
%%Inspired by the spacey principle to choose a previous type, we also propose a special ``spacey" framework : 
%Finally, considering both the higher-order Markov property and multi-orientation property, 
%we define our meta-graph based heterogeneous personalized spacey random walk as follows.
%We use the meta-graph in Figure XXX as an illustration which consists of two meta-paths and can define a second-order Markov chain, 
%while other meta-graphs are similar.

\begin{definition}\label{def:personalized_spacey_walk_metagraph}
%	{\it \textbf{Heterogeneous Personalized Spacey Random Walk for Meta-graph based Second-order Markov Chains}.
	{\it \textbf{Meta-graph based Heterogeneous Personalized Spacey Random Walk}.
		Given $M$ second-order Markov chains based on a meta-graph $\mathcal{T}_{\mathcal S} = (\mathcal A_S, \mathcal R_S)$ integrating $M$ meta-paths,
		an integrated transition hypermatrix ${\bf \overline{H}}$ for this meta-graph is defined as:
		\begin{equation}
		{\bf \overline{H}}_{i,j,k}=\frac{1}{\sum_{m} Ind \{{\bf H}_{i,j,k}^m >0\}}\sum_{m} {\bf H}_{i,j,k}^m,
		\end{equation}
		where ${\bf H}^m$ is the transition probabilities of $m$-th Markov chain as defined in Eq.~(\ref{Eq:second_order_transition_hypermatrix}).
		Then, the probability law to guide the meta-graph based heterogeneous personalized spacey random walk 
		%with a sequence of random variables $X(0), X(1), X(2),\cdots \!,X(n)$, 
		is defined to use the personalized occupation probability (as defined in Eq.~(\ref{Eq:spacey_out_law})) to choose the second last state $Y(n)$, 
		and use
		\begin{equation}\label{Eq:spacey_type}
		Pr\!\{\Phi \!(n\!+\!1)\!\!=\!\!A | X\!(n)\!\!=\!\!v_j,  \! Y\!(n)\!\!=\!\!v_i \}\! \! \triangleq \!\!
		\begin{cases}
		\!(1\!\!-\!\!\alpha)\frac{1}{|\!N_{\!{\small \mathcal{T}_{\!\mathcal S}}}\!(v_i\!,\!v_j)\!|}\!+\!\alpha {\bf z}_{\!A}\!(n),\!\!&\! \!A\!\!\in \!\! N_{\!\mathcal{T}_{\!\mathcal S}}\!(v_i\!,\!v_j) \\
		0, & otherwise
		\end{cases}
		\end{equation}
		to choose the next node type $\Phi(n+1)$, and then use
		\begin{equation}\label{Eq:spacey_walk_metagraph}
		Pr\!\left\{X\!(n\!\!+\!\!1)\!=\!v_k | X\!(n)\!=\!v_j, Y\!(n)\!=\!v_i, \Phi(n\!\!+\!\!1)\!= \!A \right\}  \!\!\triangleq \!\!
		\begin{cases}
		{\bf \overline{H}}_{i,j,k},\! & \!\phi(v_k)\!=\!A \\
		0, & \phi(v_k) \! \not =\!A
		\end{cases}
		\end{equation}
		to choose the next node, where $N_{\!{\small \mathcal{T}_{\!\mathcal S}}}\!(v_i,\!v_j)$ is the set of successor types of edge $(\phi (v_i),\phi (v_j))$
		 in $\mathcal{T}_{\!\mathcal S}$, $\phi(\cdot)$ is the node type mapping; 
		$ {\bf z}(n)$ is the partial occupation vector at step $n$:
		\begin{equation}\label{Eq:occupation_vector_metagraph}
		{\bf z}_{\!A}(n) \triangleq \frac{\sum_{\phi (v_i)=A } {\bf w}_i(n)}{\sum_{\phi (v_i)\in N_{\!{\small \mathcal{T}_{\!\mathcal S}}}\!(X\!(n),\!Y\!(n))} {\bf w}_i(n)},\ \  A\!\!\in \!\! N_{\!\mathcal{T}_{\!\mathcal S}}\!(X\!(n),\!Y\!(n)).
		\end{equation}
	}
\end{definition}
In short, with personalization, when the meta-graph based spacey random walker visits $X(n)$ at step $n$, it first forgets its second last state (i.e., the state $X(n-1)$) with a probability $\alpha$ and invents a new history state $Y(n)$ by randomly drawing a past state $X(1),...,X(n)$.
Next, if there are %multi-oriented node types, 
branched node types,
it chooses the next type $\Phi(n+1)$  according to their history distribution with probability $\alpha$.
Then it transitions to $X(n+1)$ as if its last two states were $X(n)$ and $Y(n)$ and current node type $\phi (X(n+1))$ is $\Phi(n+1)$.
Without personalization, it performs a non-spacey random walk and randomly chooses the next one from branched node types.

We develop the {\it SpaceyMetagraph} algorithm by leveraging the meta-graph based personalized spacey random walk to generate heterogeneous neighborhood, and then incorporating them to the Skipgram model to produce effective HIN embeddings.



% For example, for the APA meta-path, if we concatenate two $APA$ meta-paths to be $APAPA$, we have:
% \begin{equation}
% S(i,j) =\sum [\# {\mathrm paper_{by}}(i,k)] \cdot
% [\# {\mathrm paper_{by}}(j,k)],
% % S(i,j) =\sum [\# {\rm shared \; words \; in \; document} \; i \; {\rm and } \; k] \cdot
% % [\# {\rm shared \; words \; in \; document} \; j \; {\rm and } \; k].
% \end{equation}
% where $\# {\mathrm paper_{by}}(i,k)$ means the co-authored papers published by authors $i$ and $k$.
% This means that, if there are more co-authors (indexed as $k$) overlapped between two authors $i$ and $j$, they are more similar.
% Even though the original bipartite network structure does not have direct author-author links, we can compute it based on the author-paper links.


%\begin{figure}[t]
%    \vspace{-0.15in}
%	\includegraphics[width=0.25\textwidth]{multipath}
%    \vspace{-0.15in}
%	\caption{An example of multiple meta-path similarity for scholar network. }
%	\label{fig:metaschema-sim}
%    \vspace{-0.15in}
%\end{figure}
%
%This similarity $S^{{\mathcal P}_{A_1,A_t}, {\mathcal P}_{A_2,A_t}}(i,j)$ can lead to interesting results. 
%For example, consider P as a bridge for A, we can concatenate AP and PA to APA. Consider V as a bridge of A, we can concatenate two APV to be APVPA.
%As an example, we show a meta-schema similarity for scholar network in Figure~\ref{fig:metaschema-sim}.
%From the above examples we can see that, the meta-schema proximity guided similarities provide different topological and semantic meaning that direct meta-path similarities cannot provide.
%The path constraints in the meta-schema proximity can also be factorized using a higher-order Markov chain similar as Section~\ref{sec:meta-path-guided embedding}.
%For example, for the meta-schema similarity shown in Figure~\ref{fig:metaschema-sim}, 
%we can use APA, APV, PVP, VPA, PAP to construct a second-order Markov chain.
%Thus, meta-schema proximity guided higher-order Markov chain will have more transition probabilities.
%We can simply follow the steps in section~\ref{sec:meta-path-guided embedding} to obtain the second-order proximity guided network embedding.
%We denote this extension framework as \textit{PMSW-metaschema}.
%Then we can run personalized spacey random walk for each entity, and then find the parameterized approximate stationary distributions as Task 1 ({\bf T1}) shows.





\subsection{Meta-schema based HIN Embedding}
% \vspace{-0.05in}
\label{sec:spaceymetaschema}
Although the meta-path and meta-graph have proved to be useful to capture heterogeneous semantics in an HIN,
it is quite difficult for a non-proficient user to design appropriate meta-paths or meta-graphs.
%especially in an HIN involveing a large diversity of types, such as knowledge graph etc.
Therefore, it is considerable to extend meta-path/meta-graph  driven  embedding algorithms to a general meta-schema driven embedding algorithm.
% Given the {\it SpaceyMetagraph} algorithm introduced in Section~\ref{sec:spaceymetagraph}, 
% we have provided a principled way to develop a general meta-schema based HIN embedding model, which will be clarified in this section.
%A appropriate meta-paths driven node embedding algorithm should be as easy and effective as possible to extend to a general meta-schema driven node embedding model for users who do not provide domain-specific meta-paths.
% in this section, we further extend our spacey random walk framework to develop a general meta-schema based HIN embedding model for users who do not provide domain-specific meta-paths/meta-graphs.
Unlike a meta-path or a meta-graph, the meta-schema does not contain duplicate types. 
Thus, the meta-schema guided random walk  is a first-order Markov chain and we do not need to space out  to choose previous states.
However, similar to the meta-graph guided random walk, there is a balance issue for branch choices in a meta-schema.
%For example, for the meta-schema in Figure~\ref{Fig:A_HIN}, when we need to perform random walk from the first ``P" to another type of node, there are three independent choices: ``V", ``T'' or ``A".
Therefore, we follow the {\it SpaceyMetagraph} algorithm to %adaptively balance these multi-oriented choices, that is, we make a choice according to the occupation distribution of these multi-oriented types instead of a uniform selection.
%Formally, we 
formalize the meta-schema based heterogeneous personalized random walk as follows.

\begin{definition}\label{def:personalized_spacey_walk_metaschema}
	{\it \textbf{Meta-schema based Heterogeneous Personalized Random Walk}.
		Given an HIN ${\mathcal G} = ({\mathcal V}, {\mathcal E})$ and its meta-schema $\mathcal T_{\mathcal G} = (\mathcal A, \mathcal R)$, 
		the transition probability matrix ${\bf P}_{A_l,A_k}$ starting from type $A_l$ to type $A_k$ is defined
%		 as:
%		\begin{equation}
%		{\bf P}_{A_l,A_k} = {\bf D}_{A_l,A_k}^{-1}{\bf W}_{A_l,A_k},
%		\end{equation}
%		where  ${\bf W}_{\!A_l,A_k}\!\in \!{\mathbb R}^{|\!{\mathcal V}_{\!A_l}\!|\times |\!{\mathcal V}_{\!A_k}\!|}$ is  the adjacency matrix between nodes in types $ A_l$ and nodes in type $ A_k$,
%		and ${\bf D}_{A_l,A_k}$ is its degree matrix.
similar as Eq.~(\ref{Eq:normalized_adjacency_matrix}).
		Then, the probability law to guide the meta-schema based heterogeneous personalized random walk
		% with a sequence of random variables $X(0), X(1), X(2),\cdots \!,X(n)$,  
		is defined to use
		\begin{equation}\label{Eq:spacey_type_metaschema}
		Pr\!\{\Phi \!(n\!+\!1)\!\!=\!\!A | X\!(n)\!\!=\!\!v_i \}\! \! \triangleq \!\!
		\begin{cases}
		\!(1\!\!-\!\!\alpha)\frac{1}{|N_{\!{\small \mathcal{T}_{\!\mathcal G}}}\!(v_i\!)|}\!+\!\alpha {\bf z}_{\!A}\!(n),\!\!&\! \!A\!\!\in \!\! N_{\!\mathcal{T}_{\!\mathcal G}}\!(v_i) \\
		0, & otherwise
		\end{cases}
		\end{equation}
		to choose the next node type $\Phi(n+1)$, and then use
		\begin{equation}\label{Eq:spacey_walk_metaschema}
		Pr\!\left\{X\!(n\!\!+\!\!1)\!=\!v_j | X\!(n)\!=\!v_i, \!\Phi(n\!\!+\!\!1)\!= \!\!A \right\}  \!\!\triangleq \!\! 
		\begin{cases}
		{\bf P}_{\!\phi\!(\!v_i\!),\!A}(v_i,\!v_j),\!\! & \!\!\phi(v_j)\!\!=\!\!A \\
		0, \!\!&\!\! \phi(v_j) \!\! \not =\!\!A
		\end{cases}
		\end{equation}
		to choose the next node, where $N_{\!{\small \mathcal{T}_{\!\mathcal G}}}\!(v_i)$ is the set of adjacency types of $\phi (v_i)$
		in $\mathcal{T}_{\!\mathcal G}$; 
		$ {\bf z}(n)$ is the partial occupation vector at step $n$:
		\begin{equation}\label{Eq:occupation_vector_metaschema}
		{\bf z}_{\!A}(n) \triangleq \frac{\sum_{\phi (v_i)=A } {\bf w}_i(n)}{\sum_{\phi (v_i)\in N_{\!{\small \mathcal{T}_{\!\mathcal G}}}\!(X\!(n))} {\bf w}_i(n)},\ \  A\!\!\in \!\! N_{\!\mathcal{T}_{\!\mathcal G}}\!(X\!(n)).
		\end{equation}
	}
\end{definition}

Note that the meta-schema based heterogeneous personalized spacey random walk is a special case of the meta-graph based one where the meta-graph only has first-order Markov chains.
It is different from directly performing random walk on the HIN by treating it as a homogeneous graph, as it dynamically determines what is the type of next node and choose a random node under the chosen type.
% Given an arbitrary heterogeneous network with a meta-schema, we can use the above meta-schema based personalized random walk to generate heterogeneous node sequences without any handcrafted meta-path or meta-graph.
Given the random walk based node sequences, the Skipgram model can be used to  learn  embeddings as described in Section~\ref{sec:spaceymetapath}.
We similarly denote this general framework as  {\it SpaceyMetaschema}.



















==> v5 - for arxiv/introduction.tex <==
%\vspace{-0.1in}
\section{Introduction}\label{sec:introduction}
% Network embedding is a general and fundamental technique to represent nodes of a network as vectors in a low-dimensional space~\cite{PengCui2017,GoyalF17,HongYunCai2018}.
% %It can be used to improve a lot of real applications such as node profiling (classification or clustering)~\cite{RenEWH15,RenEWTVH15}, link prediction~\cite{KongZY13,ZhangKY13,YuRSGSKNH14,ShiZLYYW15}, similarity search~\cite{Sun2011a,SunNHYYY12}, etc.
% %Recently, with the development of more scalable machine learning systems and better optimization algorithms, network embedding has been applied to very large-scale networks, which makes it more applicable than before~\cite{PerozziAS14,TangQWZYM15,GroverL16}.
% While it has recently received a lot of research attention, 
% most of them (e.g., DeepWalk~\cite{PerozziAS14}, LINE~\cite{TangQWZYM15}, node2vec~\cite{GroverL16}) are focused on homogeneous network embedding which only treat single-typed nodes and edges.
% In the real-world applications, however, 
% a large number of networks such as modern social media~\cite{KongZY13}, scholar networks~\cite{Sun2011a}, %patient and drug networks~\cite{denny2012mining}, 
% and knowledge graphs~\cite{dong2014knowledge}, should essentially be represented as {Heterogeneous Information Networks} (HINs) where the nodes (i.e. entities) and edges (i.e. relationships) can be categorized into different types~\cite{shi2017survey}.

% For example, 
% consider a scholar network, as illustrated in Figure~\ref{Fig:A_HIN}, which consists of three entity types: {\it Author}, {\it Paper} and {\it Venue}, and two relationships:
% an author {\it writes} a paper, and a paper is {\it published} in a conference venue.
% We can introduce two meta-paths~\cite{Sun2011a}: ``{\it Author--Paper--Author} (APA)'' and ``{\it Author--Paper--Venue--Paper--Author} (APVPA)'' which measure the similarity of two authors who co-author many papers or whose papers are published at the same venues. The latter meta-path gives a more specific definition about how the two authors are seen as similar.
% Thus, if we can extract the semantics of different meta-paths using network embedding, 
% it can help with many downstream analysis for HIN-specific applications,
% such as link prediction or recommendation in HINs~\cite{YuRSGSKNH14,ZhaoYLSL17,HuSZY18}, entity typing~\cite{RenEWTVH15}, and similarity search~\cite{Sun2011a}.


{Heterogeneous Information Networks} (HINs) have been studied for several years and proven to be useful for many applications~\cite{shi2017survey,cai2018comprehensive}.
The heterogeneous information provided by the types of entities and their relationships in HINs can capture more semantically meaningful information than homogeneous networks~\cite{Sun2011a}.
For example, 
consider a scholar network, as illustrated in Figure~\ref{Fig:A_HIN}, which consists of three entity types: {\it Author}, {\it Paper}, and {\it Venue}, and two relationships: an author {\it writes} a paper, and a paper is {\it published} in a conference venue.
We can introduce two meta-paths~\cite{Sun2011a}: ``{\it Author--Paper--Author} (APA)'' and ``{\it Author--Paper--Venue--Paper--Author} (APVPA)'' which measure the similarity of two authors who co-author many papers or whose papers are published at the same venues. 
The semantics of the two meta-paths give two specific definitions about how the two authors are seen as similar.
Many HIN-specific applications, 
such as entity typing~\cite{RenEWH15,RenEWTVH15}, similarity search~\cite{Sun2011a,SunNHYYY12}, and link prediction~\cite{YuRSGSKNH14,ZhaoYLSL17,HuSZY18}, have been applied to use the semantics of different meta-paths in HINs and have been shown to be useful.


Recently, inspired by the DeepWalk algorithm for homogeneous networks~\cite{PerozziAS14}, meta-path(s) guided random walk based HIN embedding algorithms have also been developed~\cite{YuxiaoDong2017,FuLL17,ChuanShi2017,zhang2018metagraph2vec}.
In general, these algorithms use a two-step approach to generate node embeddings.
First, they perform random walks on an HIN guided by one or mutiple meta-path(s). %~\cite{LaoC10}.
Then they run a Skipgram algorithm which was invented in word embedding approach word2vec~\cite{Mikolov2013} to generate the node embeddings.
The idea of Skipgram algorithm is to use a central node to predict its context nodes given by the random-walk paths.
%and has been shown to be an implicit factorization of a specific form of node-context distribution matrix~\cite{cao2015grarep,qiu2018network}.
%Although these algorithms can handle the heterogeneity of HINs and capture semantically meaningful information provided by meta-paths,
%Although these algorithms can capture the heterogeneous information provided by meta-paths and have been shown to be beneficial to HIN-specific applications, 
Despite their success in capturing the heterogeneous information provided by meta-paths and thus learning valuable embedding vectors, 
there are still some problems.
First,
the meta-path guided random walk uses sampling to generate node paths, which are in essence sampled from a higher-order Markov chain.
For example, as illustrated in Figure~\ref{Fig:A_HIN}, for the random walks guided by the  meta-path ``APVPA'', we will constrain that  for the first ``P'' in the meta-path, the next node must be ``V'' and for the second ``P'' in the meta-path, the next node must be ``A''. That is, when we perform next walk from a ``P'', we need to know the previous state before ``P'' being ``A'' or ``V'' to judge the ``P'' being the first or the second. Thus, this is theoretically a second-order Markovian stochastic process.
% because the transition
% %depend on the last two states, rather than just the last one.
% is determined by the last two states. %rather than just the last one.
However, existing algorithms have paid few attention to the essence of the higher-order Markov chain property of meta-path guided random walk, especially to its limiting stationary distribution.
As a random walk can be regarded as a random sampling from the stationary distribution, their inattentive sampling may result in less accurate approximation of the stationary distribution and consequently may have less effective node embeddings.
%In other words, faster converged sampling chains will result in more efficient embedding algorithms.
%As a result, their random walk simulations, while generating the walk paths constrained by the meta-path, can be insensitive and inefficient to be stationary.
%Consequently, the learned emdeddings may be less reliable due to the unguaranteed stationarity of node distribution generated by insufficient random walks.
Second,
compared with single meta-path, meta-graph is able to capture richer information by integrating multiple meta-paths.
However, as different meta-paths characterize different semantics, it is still a challenge how to effectively select and balance multiple meta-paths with appropriate weights.
Moreover, 
the design of meta-paths is usually domain-specific and is difficult for a non-proficient user.
Thus, a more principled way of performing HIN embedding should be fit to extend to a general meta-schema driven embedding model for when proficient design is impracticable.


%Second, existing algorithms are sensitive to different meta-paths, which means that they need a \emph{feature engineering} step: involving domain experts to manually design domain-specific meta-paths.
%Obviously, it is quite difficult for a non-proficient user to use these algorithms, especially in HINs with tremendous variety of types, such as a knowledge graph.
%An appropriate way of performing HIN embedding is preferred as easy and effective as possible to extend to a general meta-graph or meta-schema driven embedding model for users without domain-specific meta-paths.
%Third, they only consider meta-paths with same start and end entity types. Although it may be able to claim that the random walk can be generalized to arbitrary meta-paths, there has been no principled way to do it.
\begin{figure}
	\small
	\setlength{\abovecaptionskip}{-0.1cm}
	\setlength{\belowcaptionskip}{-0.5cm}
	\centering
	\includegraphics[width=0.5\textwidth]{resources/A_HIN}
	\caption{\small An illustrative  heterogeneous scholar network with three entity types: {\it Author}(A), {\it Paper}(P), and {\it Venue}(V), as well as  its meta-schema and some meta-paths/meta-graphs on the meta-schema.}
	\label{Fig:A_HIN}
	\vspace{-0.2cm}
\end{figure}


In this paper, to address the above issues, first,
we  systematically clarify that the meta-path guided random walk is a higher-order Markov chain process.
Then a meta-path based heterogeneous personalized spacey random walk (called {\it HeteSpaceyWalk}) is introduced to improve the walk effectiveness and efficiency by leveraging a non-Markovian spacey strategy.
Given an arbitrary meta-path,
instead of strictly constraining the walks by the meta-path,
the {\it HeteSpaceyWalk} allows spacing out and skipping the intermediate trivial transitions, and in fact performs a special meta-graph guided random walk, which differs from the normal one in four aspects: 
(a) The special meta-graph integrates multiple meta-paths which are automatically produced by folding the original user-given meta-path.
(b) The trade-off of these integrated meta-paths are dynamically self-adjusted. That is, during the walk process, {\it HeteSpaceyWalk} adaptively adjusts the probability of following each possible meta-path according to the carefully designed personalized spacey strategy.
(c) {\it HeteSpaceyWalk} is mathematically guaranteed to attain the same unique limiting stationary distribution with the original meta-path guided higher-order Markovian random walk.
(d) By spacing out and skipping the intermediate trivial transitions, {\it HeteSpaceyWalk} provides a cost-efficient sampling way to be stationary and thus can produce more effective embeddings with less walk-times and walk-length than original meta-path constrained random walk sampling.



Second, by leveraging the {\it HeteSpaceyWalk} process to generate heterogeneous neighborhood, and incorporating them to the Skipgram model, 
we develop a general scalable HIN embedding algorithm: {\it SpaceyMetapath}, which is able to produce semantically meaningful embeddings for multi-typed nodes in an HIN with an arbitrary user-given meta-path.
Further, we extend the guidance from a single meta-path to a user-given meta-graph and a general non-handcrafted meta-schema, and develop two embedding algorithms:  {\it SpaceyMetagraph} and  {\it SpaceyMetaschema}.
The main contributions of our work are summarized as follows:
%We summarize our main contributions as follows:

%we propose to use a higher-order Markov-chain based random walk to guide the HIN embeddings process.
%By formulating the higher-order Markov chain defined by the types of entities and their relationships, we design a personalized spacey random walk to obtain the expected (stationary) commute time distribution among nodes, and then use a set of embedding vectors to approximate the commute time among nodes.
%The embedding vectors will then represent the semantics guided by an arbitrary meta-path provided by a user.
%We then extend the guidance from a single meta-path to multiple meta-paths corresponding to the second-order proximities in the network meta-schema of the HIN.
%The embeddings will then be a semantic representation of an ensemble of multiple paths.

% We propose to use a {higher-order Markov chain} to represent arbitrary meta-paths, which is based on solid and elegant mathematical foundation~\cite{BensonGL17}.
% Then the HIN embedding is learned from the stationary distributions of the personalized random walk based on the higher-order Markov chain.
% Based on this framework, we further propose HIN embedding guided by second-order meta-schema proximity which involves more than one meta-path


% Compared to conventional homogeneous network embedding models\cite{PerozziAS14,TangQWZYM15,GroverL16}, the proposed high-order Markov chain based random walk models are effective to handle the diversity of node types and relationship types and thus introduce the higher-level semantics of different entities and relationships to HIN embedding.
% Compared to previous HIN embedding approaches~\cite{YuxiaoDong2017,HuangM17,ShangQLKHP16}, the proposed methods can construct a high-order Markov chain based random walk guided by a arbitrary meta-path, can be formulated as an elegant objective function.
% We can also extend the higher-order Markov chain based random walk framework from a human-given meta-path to multiple meta-paths corresponding to second-order proximities in the network meta-schema of the HIN, which is quite useful to lightly relying on prior knowledge and experiences of domain experts to manually design domain-specific meta-paths.
% Moreover, the second-order meta-schema proximity guided similarities can provide different topological and semantic meaning that direct meta-path similarities cannot provide.






% We introduce to use a {higher-order Markov chain} to represent an arbitrary meta-path, which is based on solid and elegant mathematical foundation~\cite{BensonGL17}.
$\bullet$ Existing approaches have paid few attention to the higher-order Markov chain nature of meta-path guided random walk, especially to its stationary distribution.
We formalize the meta-path guided random walk as a higher-order Markov chain process, and present a heterogeneous personalized spacey random walk to efficiently and effectively attain the expected stationary distribution among nodes, which is based on a solid mathematical foundation~\cite{BensonGL17}.


$\bullet$ We propose a generalized framework for heterogeneous spacey random walk for a meta-path based higher-order Markov chain for HIN embeddings.
Based on this framework, we further extend to an arbitrary meta-graph integrating multiple meta-paths and a general
meta-schema without any handcrafted meta-paths.


$\bullet$ We use extensive experiments in four heterogeneous networks to demonstrate that the proposed methods considerably outperform both conventional homogeneous embedding and heterogeneous meta-path/meta-graph guided embedding methods in two HIN mining tasks, i.e., node classification and link prediction.

The code is available at \url{https://github.com/HKUST-KnowComp/HeteSpaceyWalk}.

% In the rest of this paper, we first introduce the related concepts of HIN in Section~\ref{sec:problem-definition}.
% Then, in Section~\ref{sec:frameworks}, we present the proposed heterogeneous personalized spacey random walk based HIN embedding frameworks, including the arbitrary meta-path based HIN embedding, arbitrary meta-graph based HIN embedding, and the general meta-schema based HIN embedding.
% Then, we show experimental results and analysis in Section~\ref{sec:experiments}.
% Finally, we review the related work in
% Section~\ref{sec:related-work} and conclude the paper in Section~\ref{sec:conclu}.



==> v5 - for arxiv/relatedwork.tex <==
\section{Related Work}\label{sec:related-work}
% Network representation learning can be categorized into latent factor models~\cite{Yan2006Graph,Hoff2002Latent,Koren2008Factorization,Ma2011Recommender} and generalized neural network-based models~\cite{PerozziAS14,GroverL16,TangQWZYM15}.
% The latent factor models are effected by application tasks, such as recommendation systems~\cite{Koren2008Factorization,Ma2011Recommender},
% node profiling (classification or clustering)~\cite{RenEWH15,RenEWTVH15}, 
% link prediction~\cite{KongZY13,ZhangKY13,YuRSGSKNH14,ShiZLYYW15}, 
% similarity search~\cite{Sun2011a,SunNHYYY12} for network analysis and graph mining.
% These models focus on factorizing the matrix/tensor format of a network, and generating latent-dimension features for nodes or edges in this network.
% However, the computational cost of decomposing a large-scale matrix/tensor is usually very expensive, and also suffers from its target function limitations, making it neither practical nor effective for addressing other tasks in big networks.
% The neural network-based network representation learning models either make use of random walk technologies generating sequence of vertex in a network, or exploit first-order and second-order proximity functions jointly to preserve the network structure.
% Bryan Perozzi et al. proposed a truncated random walk to transform the static network into a sample collection of linear sequences.
% Then use the skip-gram on hierarchical softmax function to train vertex representations.
% Grover and Leskovec et al. further generalized a biased random walkers with Breadth-First Search (BFS) and Depth-First Search (DFS) over a network, and employed the popular skip-gram with negative sampling to train vertex representations.
% Tang et al. modeled a node's context into first-order and second-order proximity\citet{TangQWZYM15}, and employs the skip-gram with negative sampling to solve the limitation of stochastic gradient descent on weighted edges without compromising the efficiency.
% Even, it was further developed into a semi-supervised model PTE for embedding text data\cite{Tang2015PTE}.
% All the above models assume that the graph has homogeneous type of nodes.
% Brand firstly introduced a heterogeneous information based random walk for recommendation problem~\cite{Brand2005A}.
% Yuxiao Dong proposed two meta-path-based random walks to construct the heterogeneous neighborhood
% of a node and then leverages a heterogeneous skip-gram model to perform node embeddings~\cite{YuxiaoDong2017}.
 
%\subsection{Heterogeneous Information Networks}
In the past decade,
%heterogeneous information network (HIN) has been extensively studied %its ubiquity in real-world data.
%for various of applications, such as entity typing (classification or clustering)~\cite{RenEWH15,RenEWTVH15}, recommendation~\cite{ZhaoYLSL17,HuSZY18}, and similarity search~\cite{Sun2011a,SunNHYYY12}.
to marry the advantages of HIN and network embedding, 
embedding learning in an HIN has received increasing attention and many heterogeneous embedding algorithms have been proposed~\cite{Bordes2013,Tang2015PTE,chang2015heterogeneous,YuxiaoDong2017,zhang2018carl,kralj2018hinmine,qiu2018network,sun2018joint,shi2018easing}.




%Different from homogeneous networks, HINs' nodes and edges have types~\cite{ShiLZSY17}.
%The major difference between an HIN and traditional graphs or networks is that an HIN has multi-typed entities and relations, and thus can provides more semantically meaningful information~\cite{ShiLZSY17}.
%Therefore, as a general and fundamental technique for network analysis and graph mining, HIN embedding have received an increasing attention.
%In general,the problems solved within HINs can be categorized in to three types: entity typing (classification or clustering)~\cite{RenEWH15,RenEWTVH15}, link prediction (homogeneous such as anchor link prediction~\cite{KongZY13} and new user prediction~\cite{ZhangKY13} or heterogeneous links such as recommendation system~\cite{YuRSGSKNH14,ShiZLYYW15}), and similarity search~\cite{Sun2011a,SunNHYYY12}.
%The analysis of an HIN is naturally related to higher-order analysis of homogeneous networks.
%For example, the meta-graph (or meta-structure)~\cite{FangLZWCL16,HuangZCSML16,HeJiang2017,HuanZhao2017} defined on HIN is similar to motifs used for homogeneous networks~\cite{milo2002network,benson2016higher}. The difference is that the meta-graph has different node types.
%In other words, a meta-graph can be considered as a motif with constraints that the nodes and edges in the motif should follow different types in the HIN meta-graph (or meta-structure).

% HINs were originally developed for analyzing scientific publication networks~\cite{Yizhou11,SunNHYYY12}.
% Today, social media analysis also uses HIN for user similarity analysis and link prediction~\cite{KongZY13,ZhangKY13,ZhangKY14}.
% Clearly the knowledge in knowledge graphs like Freebase~\cite{freebase} and Google Knowledge Vault~\cite{dong2014knowledge} can be represented as HINs, and document similarity measurement can be improved based on the knowledge graph information~\cite{Wang2015IWK,WangChenguangICDM2015,WangSLZH16}.
% More recently, mobile malware has also been found that can be formulated as an HIN allowing the derivation of multiple semantically meaningful similarities to improve mobile security~\cite{ShifuHou2017}.



%{\bf Higher-order HIN embedding: existing approaches.}
In general,
there have been multiple ways to represent multi-typed nodes in an HIN.
A straightforward method is to directly perform matrix/tensor factorization~\cite{MaruhashiGF12,PapalexakisFS17,qiu2018network} to extract vector representations of nodes. 
For example, 
{\it Collective matrix factorization} of multi-type relational data~\cite{Singh2008,NickelTK12,BouchardYG13} treats each binary relation as a matrix, and performs joint matrix factorization over different relations.
%One entity can be related by different types of entities but has only on vector representation.
%If we combine the co-occurrences of entities in binary relations (e.g., three or more types of entities such as author, paper, and venue can co-occur together), we can also use {\it tensor factorization}~\cite{MaruhashiGF12,PapalexakisFS17} to extract vector representations of entities.
However, such a way is usually costly for computation and memory.
More recently, researchers apply stochastic optimization to optimize simple or deep models to predict the binary relations between two types of entities with large-scale knowledge graphs~\cite{Nickel0TG16}.
Representative approach include {TransE}~\cite{Bordes2013} where one entity in a type is translated by a relation vector to another entity in another type given the co-occurrence of a binary relations between them and PTE~\cite{Tang2015PTE} which decomposes an HIN to a set of bipartite networks by edge types, and learns node vectors by capturing 1-hop neighborhood of the resulting bipartite networks.
All of these methods, although sometimes called higher-order factorization or embedding, are still dealing with the co-occurrence of binary relations among entities~\cite{Nickel0TG16}.
More recently, inspired by the DeepWalk model for homogeneous networks~\cite{PerozziAS14}, meta-paths or meta-graphs guided random walk based entity embedding models have also been well developed~\cite{shang2016meta,YuxiaoDong2017,FuLL17,ChuanShi2017,zhang2018metagraph2vec} using the Skipgram techniques introduced by word2vec~\cite{Mikolov2013} for very large graphs.
However, as discussed in Section~\ref{sec:introduction}, 
these algorithms have few attention on the higher-order Markov chain nature of meta-path guided random walk.
%especially on its convergent stationarity.
%and thus may suffer from the non-stationary issue. % which can result in unreliable embeddings.
%the start and end entities in the random walk are constrained to be of the same type, and direct application of random walk may cause the non-stationary distribution for certain types of meta-paths~\cite{HeJiang2017}. 
%Moreover, \cite{HuangM17,ShangQLKHP16} proposed to directly use the proximity computed by PRA's ad-hoc first hitting time probability as an HIN proximity to generate the HIN embeddings, which can be seen as a special truncated case of our stationary approximation.
%In contrast, our approach not only addresses the non-stationary issue but also generalizes to allow multiple meta-paths and the start and end entities in the random walk to be different.  
Following random walk based embedding algorithms, we focus on the higher-order Markov chains and design a new meta-path/meta-graph guided random walk strategy, and further develop several general scalable HIN embedding models.



